How Fine-Tuning Allows for Effective Meta-Learning

Representation learning has been widely studied in the context of meta-learning, enabling rapid learning of new tasks through shared representations. Recent works such as MAML have explored using fine-tuning-based metrics, which measure the ease by which fine-tuning can achieve good performance, as proxies for obtaining representations. We present a theoretical framework for analyzing representations derived from a MAML-like algorithm, assuming the available tasks use approximately the same underlying representation. We then provide risk bounds on the best predictor found by fine-tuning via gradient descent, demonstrating that the algorithm can provably leverage the shared structure. The upper bound applies to general function classes, which we demonstrate by instantiating the guarantees of our framework in the logistic regression and neural network settings. In contrast, we establish the existence of settings where any algorithm, using a representation trained with no consideration for task-specific fine-tuning, performs as well as a learner with no access to source tasks in the worst case. This separation result underscores the benefit of fine-tuning-based methods, such as MAML, over methods with "frozen representation" objectives in few-shot learning.

==> results/linear/hardcase/ermLearnsWrongSpace.tex <==
\begin{restatable}[\frzrep{} learns incorrect space]{lemma}{ermLearnsWrongSpace}
  \label{lemma:erm-learns-wrong-space}
  Fix an orthogonal matrix $B^\ast \in \reals^{d \times k}$ with $\col{B^\ast} \subseteq E^\ast$, and assume that we sample task weights from the distribution in \eqnref{eqn:lin-hard-task-dist}.
  Then, with infinitely many tasks and per-task samples $(n_\source, T \to \infty)$, $\col{\hat{B}} = E_k$.
\end{restatable}
\begin{proof}
  Fix a $B$.
  For any $t \in [T]$, as $n_\source \to \infty$, we have that
  \begin{align*}
    \min_{w_t}\frac{1}{n_\source}\norm[2]{y_t - X_tBw_t}^2 &= \min_{w_t}\frac{1}{n_\source}\norm[2]{X_t(\theta_t^\ast - Bw_t) + z_t} \\
      &= \min_{w_t}\norm[2]{\Sigma^{1/2}(\theta_t^\ast - Bw_t)}^2 + \sigma^2 \\
      &= \norm[2]{P_{\Sigma^{1/2}B}^\perp\Sigma^{1/2}\theta_t^\ast}^2 + \sigma^2.
  \end{align*}
  Therefore, we can rewrite the objective defining $\hat{B}$ as
  \begin{align*}
    \hat{B} &= \argmin_{B}\frac{1}{T}\sum_{t \in [T]}\norm[2]{P_{\Sigma^{1/2}B}^\perp\Sigma^{1/2}\theta_t^\ast}^2 \\
      &= \argmin_{B}\tr P_{\Sigma^{1/2}B}^\perp\Sigma^{1/2}\left[\frac{1}{T}\sum_{t \in [T]}\theta_t^\ast(\theta_t^\ast)^\top\right]\Sigma^{1/2} \\
      &= \argmin_{B}\tr P_{\Sigma^{1/2}B}^\perp\left[\frac{1}{2}P_{B^\ast} + P_{E_k}\right] \\
      &= \argmin_{B}\frac{1}{2}\norm[F]{P_{\Sigma^{1/2}B}^\perp P_{B^\ast}}^2 + \norm[F]{P_{\Sigma^{1/2}B}^\perp P_{E_k}}^2,
  \end{align*}
  where the third equality uses the definition of the task distribution in \eqnref{eqn:lin-hard-task-dist}.
  Now, let $S$ be the space defined as $E_k + \mathrm{Col} \ B^\ast$.
  Observe that
  \begin{align*}
    \norm[F]{P_{\Sigma^{1/2}B}^\perp P_S}^2 &= \tr{P_{\Sigma^{1/2}B}^\perp P_S} \\
      &= \tr{P_{\Sigma^{1/2}B}^\perp P_B^\ast} + \tr{P_{\Sigma^{1/2}B}^\perp P_{E_k}} \\
      &= \norm[F]{P_{\Sigma^{1/2}B}^\perp P_{B^\ast}}^2 + \norm[F]{P_{\Sigma^{1/2}B}^\perp P_{E_k}}^2.
  \end{align*}
  By putting everything together, we thus see that
  \[
    \hat{B} = \argmin_{B}\norm[F]{P_{\Sigma^{1/2}B}^\perp P_{S}}^2 + \norm[F]{P_{\Sigma^{1/2}B}^\perp P_{E_k}}^2.
  \]
  This objective is minimized if and only if the span of $\Sigma^{1/2}B$ is exactly $E_k$.
  By inverting, this is only possible if $\mathrm{Col} \ \hat{B} = E_k$.
\end{proof}


==> results/linear/hardcase/ermMinimaxBound.tex <==
\begin{restatable}[\frzrep{} minimax bound]{theorem}{ermMinimaxBound}
  \label{thm:erm-minimax-bound}
  \IfAppendix{
    For an orthogonal matrix $B^\ast \in \reals^{d \times k}$ whose column space lies in $E^\ast$, let $S_{B^\ast}$ be the set
    \[
      S_{B^\ast} \defas \set{\frac{1}{\sqrt{2\epsilon}}B^\ast w + \delta \suchthat \norm[2]{w} \leq 1, \norm[2]{\delta} \leq 1, \delta \in E_k}.
    \]
    We consider the following procedure:
    \begin{enumerate}
      \item We draw $n_\target$ samples for target time training, which are collected into a matrix $X$.
      \item Player chooses a target-time estimator $\hat\theta = \bar{B}\hat{w} + \hat\delta$, where $\bar{B}$, $\hat{w}$, and $\hat\delta$ are measurable function of $(X, y)$, and $\col{\bar{B}} = \col{\hat{B}}$.
      \item Player chooses target-time estimator $\hat\theta = \hat{B}\hat{w} + \hat\delta$, where $\hat{w}$ and $\hat\delta$ are measurable functions of $(\hat{B}, X, y)$.
      \item Adversary chooses an orthogonal matrix $B^\ast \in \reals^{d \times k}$ satisfying $\col{B^\ast} \subset E_k$, and a target time predictor $\theta^\ast \in S_{B^\ast}$.
      \item \frzrep{} returns a representation $\hat{B}$ under the setting of \lemmaref{lemma:erm-learns-wrong-space} with the task distribution determined by $B^\ast$.
      \item Target time samples are generated using $y \sim \gaussian{X\theta^\ast, \sigma^2I_n}$, and the player estimator is evaluated.
    \end{enumerate}
    Then, with probability at least $1 - \delta$ over the draw of $X$, we have that
    \[
      \min_{\hat{w}, \hat{\delta}}\max_{\substack{B^\ast \\ \theta^\ast \in S_{B^\ast}}}\expt{\frac{1}{n_T}\norm[2]{X(\theta^\ast - \hat{B}\hat{w} - \hat{\delta})}^2} \gtrsim \frac{\sigma^2 d}{n_T},
    \]
    where the expectation is over the randomness in the labels $y \sim \gaussian{X\theta^\ast, \sigma^2 I_{n_\target}}$.
    Note that the minimization over $\hat{w}$ and $\hat{\delta}$ is performed over the set of measurable functions from $(X, y)$ to $\reals^k$ and $\reals^d$, respectively.
  }{
    For an orthogonal matrix $B^\ast \in \reals^{d \times k}$ whose column space lies in $E^\ast$, let $S_{B^\ast}$ be the set
    \[
      S_{B^\ast} \defas \set{\frac{1}{\sqrt{2\epsilon}}B^\ast w + \delta \suchthat \norm[2]{w} \leq 1, \norm[2]{\delta} \leq 1, \delta \in E_k}.
    \]
    Then, with high probability over the draw of $n_T \gg d$ samples during target training, we have that
    \[
      \min_{\substack{\bar{B}, \hat{w}, \hat{\delta} \\ \col{\bar{B}} = \col{\hat{B}}}}\max_{\substack{B^\ast \\ \theta^\ast \in S_{B^\ast}}}\expt{\frac{1}{n_T}\norm[2]{X(\theta^\ast - \bar{B}\hat{w} - \hat{\delta})}^2} \gtrsim \frac{\sigma^2 d}{n_T},
    \]
    where $\hat B$ is the output of \frzrep{} in the setting of \lemmaref{lemma:erm-learns-wrong-space}, with the task distribution determined by $B^\ast$.
    The expectation is over the randomness in the labels $y \sim \gaussian{X\theta^\ast, \sigma^2 I_{n_\target}}$.
    Furthermore, $\bar{B}$, $\hat{w}$, and $\hat\delta$ are measurable functions of $(X, y)$ to $\reals^{d \times k}, \reals^k,$ and $\reals^d$, respectively.
  }
\end{restatable}
\begin{proof}
  We instantiate the event guaranteed by \lemmaref{lemma:lin-targ-cov-concentration} over the draw of target samples, which guarantees that
  \[
    0.9\Sigma \lesssim \frac{1}{n_T}X^\top X \lesssim 1.1\Sigma,
  \]
  with probability at least $1 - \delta$.

  Recall that by \lemmaref{lemma:erm-learns-wrong-space}, \frzrep{} will always find an orthogonal matrix whose column space is $E_k$, no matter how $B^\ast$ is chosen.
  Therefore, we can rewrite the minimax expression as
  \begin{align*}
    \min_{\hat{w}, \hat{\delta}}\max_{\substack{B^\ast, \theta^\ast \\ \theta^\ast \in S_{B^\ast}}}\expt{\frac{1}{n_T}\norm[2]{X(\theta^\ast - \hat{B}\hat{w} - \hat{\delta})}^2} &= \min_{\hat\theta}\max_{\substack{B^\ast, \theta^\ast \\ \theta^\ast \in S_{B^\ast}}}\expt{\frac{1}{n_T}\norm[2]{X(\theta^\ast - \hat\theta)}^2} \\
      &\gtrsim \min_{\hat\theta}\max_{\substack{B^\ast, \theta^\ast \\ \theta^\ast \in S_{B^\ast}}}\expt{\norm[\Sigma]{\theta^\ast - \hat\theta}^2},
  \end{align*}
  where $\hat\theta$ is simply a measurable function of $(X, y)$ to $\reals^d$.
  To further simplify the problem, observe that if we define the set
  \[
    T = \set{\theta \in \reals^d \suchthat \norm[2]{P_{E^\ast}\theta}^2 \leq \frac{1}{2\epsilon}, \norm[2]{P_{E_k}\theta}^2 \leq 1} \subseteq S_{B^\ast}
  \]
  then since the estimator only depends on $B^\ast$ through $\theta^\ast$,
  \begin{equation}
    \label{eqn-int:minmax-in-signorm}
    \min_{\hat{w}, \hat{\delta}}\max_{\substack{B^\ast, \theta^\ast \\ \theta^\ast \in S_{B^\ast}}}\expt{\frac{1}{n_T}\norm[2]{X(\theta^\ast - \hat{B}\hat{w} - \hat{\delta})}^2} \gtrsim \min_{\hat\theta}\max_{\theta^\ast \in T}\expt{\norm[\Sigma]{(\theta^\ast - \hat\theta)}^2}.
  \end{equation}

  To lower bound the right-hand side of \eqnref{eqn-int:minmax-in-signorm}, we use local coverings in the $\Sigma$-norm and apply the Fano bound for minimax risk.
  Let $B \defas \set{\theta \in \reals^d \suchthat \epsilon\norm[2]{P_{E^\ast}\theta}^2 + \norm[2]{P_{E_k}\theta}^2 \leq 1}$ be the unit ball in the $\Sigma$-norm, so that $\frac{1}{\sqrt{2}}B \subseteq T$.
  Using a known volumetric argument, there exists a $(1/2)$-packing of $B$ in the $\Sigma$-norm with at least $2^d$ elements.
  Equivalently, there exists a $2\delta$-packing of $4\delta B$ with at least $2^d$ elements -- let this packing be $S$.
  Then, for any $\theta, \theta' \in S$,
  \begin{align*}
    \KL{\gaussian{X\theta, \sigma^2I_{n_T}}}{\gaussian{X\theta', \sigma^2I_{n_T}}} &= \frac{1}{2\sigma^2}\norm[2]{X(\theta - \theta')}^2 \lesssim \frac{n_T}{2\sigma^2}\norm[\Sigma]{\theta - \theta'}^2 \\
      &\leq \frac{32n_T}{\sigma^2}\delta^2.
  \end{align*}
  Therefore, by Fano's inequality, for any $\delta^2 \leq 1/32$ (which ensures that $S \subseteq 4\delta B \subseteq \frac{1}{\sqrt{2}}B \subseteq T$),
  \begin{align*}
    \min_{\hat\theta}\max_{\theta^\ast \in T}\expt{\frac{1}{n}\norm[\Sigma]{(\theta^\ast - \hat\theta)}^2} &\geq \delta^2\left(1 - \frac{32n}{\sigma^2d\log 2}\delta^2 - \frac{1}{d}\right) \\
      &\geq \delta^2\left(\frac{3}{4} - \frac{32n}{\sigma^2 d\log 2}\delta^2\right). && (d \geq 4)
  \end{align*}
  As long as $n_T \geq \frac{\log 2}{2}\sigma^2 d$, we can set $\delta^2 = \left(\frac{\log 2}{64}\right)\frac{\sigma^2d}{n_T}$, and thus putting everything together, we have that
  \[
    \min_{\hat{w}, \hat{\delta}}\max_{\substack{B^\ast, \theta^\ast \\ \theta^\ast \in S_{B^\ast}}}\expt{\frac{1}{n}\norm[2]{X(\theta^\ast - \hat{B}\hat{w} - \hat{\delta})}^2} \gtrsim \frac{\sigma^2 d}{n_T}. \qedhere
  \]
\end{proof}


==> results/linear/perf/linApproxLinearity.tex <==
\begin{restatable}[Approximate linearity of function class]{lemma}{linApproxLinearity}
  \label{lemma:lin-approx-linearity}
  Let $g_{\theta}(x) = \beta x^\top(A_{B_0} + \Delta)(w_0 + w)$ for $\theta = (\Delta, w) \in \constraintset_\beta$, where $\constraintset_\beta$ is considered as a subset of $\reals^{dk + k}$.
  Then, assuming the high-probability event in \lemmaref{lemma:lin-targ-cov-concentration} holds, then
  \[
    \sup_{\theta \in \constraintset_\beta}\frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]^2g_\theta(x_i)}^2 \lesssim \beta^2\tr\Sigma \quad \text{and} \quad \frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]g_0(x_i)}^2 \lesssim \beta^2\tr\Sigma.
  \]
\end{restatable}
\begin{proof}
  To bound the average squared Hessian operator norm, note that $\grad[\theta]^2g_\theta(x_i)[\Delta, w] = \beta x_i^\top\Delta w$, which is independent of $\theta$.
  Then, by the variational characterization of the operator norm,
  \begin{align*}
    \norm[2]{\grad[\theta]^2g_\theta(x_i)} &= \sup_{\norm[F]{\Delta}^2 + \norm[2]{w}^2 \leq 1}\abs{\grad[\theta]^2g_\theta(x_i)[\Delta, w]} = \sup_{\norm[F]{\Delta}^2 + \norm[2]{w}^2 \leq 1}\beta\abs{x_i^\top \Delta w} \\
      &\leq \sup_{\norm[F]{\Delta}^2 + \norm[2]{w}^2 \leq 1}\beta\norm[2]{x_i}\norm[F]{\Delta}\norm[2]{w} \\
      &\leq \beta\norm[2]{x_i}.
  \end{align*}
  and thus $\norm[2]{\grad[\theta]^2 g_\theta(x_i)}^2 \lesssim \beta^2\norm[2]{x_i}^2$.
  Consequently,
  \[
    \sup_{\theta \in \constraintset_\beta}\frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]^2 g_\theta(x_i)}^2 \leq \frac{\beta^2}{n_\target}\tr XX^\top \lesssim \beta^2\tr\Sigma.
  \]

  We now proceed to bound the squared norm of the gradient.
  Observe that the gradient is given by $\grad[\theta]g_0(x_i) = \beta[A_{B_0}^\top x_i, \mathrm{vec}(x_iw_0^\top)]$, and therefore,
  \begin{align*}
    \frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]g_0(x_i)}^2 &= \frac{\beta^2}{n_\target}\sum_{i \in [n_\target]}\norm[2]{A_{B_0}^\top x_i}^2 + \norm[F]{x_iw_0^\top}^2 \lesssim \frac{\beta^2}{n_\target}\sum_{i \in [n_\target]}\norm[2]{x_i}^2 = \frac{\beta^2}{n_\target}\tr XX^\top \\
      &\lesssim \beta^2\tr\Sigma,
  \end{align*}
  where the first inequality uses the fact that $\norm[2]{A^\top_{B_0}x_i}^2 = 2\norm[2]{B_0^\top x_i}^2 = 2\norm[2]{P_{B_0}x_i}^2 \lesssim \norm[2]{x_i}^2$, by the definition of $A_{B_0}$ and assumed orthogonality of $B_0$.
\end{proof}


==> results/linear/perf/linLipLoss.tex <==
\begin{restatable}[$\meanloss_\beta$ is Lipschitz]{lemma}{linLipLoss}
  \label{lemma:lin-lip-loss}
  Let $g_{\theta}(x) = \beta x^\top(A_{B_0} + \Delta)(w_0 + w)$ for $\theta = (\Delta, w) \in \constraintset_\beta$, where $\constraintset_\beta$ is considered as a subset of $\reals^{dk + k}$.
  Furthermore, assume that the high-probability event in \lemmaref{lemma:lin-targ-cov-concentration} holds.
  Then, with probability at least $1 - \delta/3$ over the draw of $n_\target$ labels, we have that for any $c_1, c_2 > 0$ and $\beta^2 > c_1^2 + c_2^2$,
  \[
    \sup_{\theta \in \constraintset_\beta}\norm[2]{\grad[g]\meanloss_\beta(g_\theta(X))}^2 \lesssim \frac{1}{n_\target}\left[\norm[2]{\Sigma}\left(\norm[2]{\theta^\ast}^2 + c_1^2 + c_2^2\right) + \sigma^2\left(1 + \log\frac{1}{\delta}\right)\right].
  \]
\end{restatable}
\begin{proof}
  We assume that $\norm[2]{z}^2/n_\target \lesssim \sigma^2[1 + \log(1/\delta)]$, which occurs with probability at least $1 - \delta/3$ via standard tail bounds on chi-squared random variables.
  Then, the gradient of the loss with respect to the predictions is given by
  \[
    \grad[g]\meanloss_\beta(g_\theta(X)) = \frac{1}{n_\target}(y - g_\theta(X)) = \frac{1}{n_\target}[X(\theta^\ast - \beta A_{B_0}w - \beta\Delta w_0 - \beta\Delta w) + z].
  \]
  Therefore,
  \begin{align*}
    \sup_{\theta \in \constraintset_\beta}\norm[2]{\grad[g]\meanloss_\beta(g_\theta(X))}^2 &\lesssim \sup_{\theta \in \constraintset_\beta}\frac{1}{n_\target^2}\norm[2]{X(\theta^\ast - \beta A_{B_0}w_0 - \beta\Delta w_0 - \beta\Delta w)}^2 + \frac{1}{n_\target^2}\norm[2]{z}^2 \\
      &\lesssim \frac{1}{n_\target}\left[\norm[2]{\Sigma}\left(\norm[2]{\theta^\ast}^2 + c_1^2 + c_2^2\right) + \sigma^2\left(1 + \log\frac{1}{\delta}\right)\right]. \qedhere
  \end{align*}
\end{proof}


==> results/linear/perf/linMainResult.tex <==
\begin{restatable}[Performance guarantee, linear representations]{theorem}{linMainResult}
  \label{thm:lin-case-main-result}
  Fix a failure probability $\delta \in (0, 1)$.
  Assume that \Cref{assump:sg-inputs,assump:lin-diversity-cond} hold, and that $n_\source \gg \rho^4(d + \log(T/\delta))$ and $n_\target \gg \rho^4(d + \log(1/\delta))$.
  Then there are $(\lambda, \gamma, \beta, T_{\pgd}, \eta, c_1, c_2)$ \IfAppendix{}{(specified in \secref{sec:lin-case-proof})} such that with probability at least $1 - \delta$ over the random draw of all samples, the training procedure in \secref{sec:lin-training-procedure} can find a parameter $\theta$ such that the excess risk on the target task is bounded by
  \[
    \IfAppendix{
      \expt{(x^\top\theta^\ast - x^\top\theta)^2} \lesssim \min(r_\target^{(1)}(n_\target), r_\target^{(2)}(n_\target), r_\target^{(3)}(n_\target)).
    }{
      \expt{(x^\top\theta^\ast - x^\top\theta)^2} \lesssim \min\left(r_\target^{(1)}(n_\target), r_\target^{(2)}(n_\target), \frac{\sigma^2d}{n_\target}\right).
    }
  \]
\end{restatable}
\begin{proof}
  Assume that during source training, the regularization parameters $(\lambda, \gamma)$ are chosen according to \lemmaref{lemma:lin-source-train-bound}.
  We instantiate the high-probability events in \Cref{lemma:lin-source-train-bound,lemma:lin-targ-stat-rates,lemma:lin-lip-loss}.
  These events occur altogether with probability at least $1 - \delta$.
  Throughout the proof, we define $r(n) = \min(r_\target^{(1)}(n), r_\target^{(2)}(n), r_\target^{(3)}(n))$.

  Given all the events above, we know that the optimization landscape induced by $\meanloss_\beta$ is well-behaved.
  That is, the function class is approximately linear in the parameters by \lemmaref{lemma:lin-approx-linearity} and the loss is Lipschitz by \lemmaref{lemma:lin-lip-loss}.
  Furthermore, for any of the proposed feasible sets in \lemmaref{lemma:lin-targ-stat-rates}, the bounds on relevant quantities provided by \lemmaref{lemma:lin-opt-consts} imply that
  \[
    c_1^2 + c_2^2 \lesssim \underbrace{\kappa(\norm[2]{B^\ast w^\ast}^2 + \delta_0^2)}_{\asdef R^2} \implies \sup_{\theta \in \constraintset_\beta}\norm[2]{\grad[g]\meanloss_\beta(g_\theta(X))}^2 \lesssim \frac{1}{n_\target}\underbrace{\left[\norm[2]{\Sigma}R^2 + \sigma^2\left(1 + \log\frac{1}{\delta}\right)\right]}_{\asdef \alpha^2}.
  \]
  Therefore, we have demonstrated that $\meanloss_\beta$ satisfies the assumptions in \secref{sec:pgd-performance-bound} for any $\beta > R^2$.
  Consequently, by running projected gradient descent with parameters
  \[
    \beta = \max\left(R^2, \frac{\alpha R^2\sqrt{\tr\Sigma}}{r(n_\target)}\right) \quad \text{and} \quad T_\pgd = \frac{\alpha^2R^2\tr\Sigma}{r(n_\target)^2},
  \]
  and setting $\eta$ as in \thmref{thm:pgd-performance-bound}, we can guarantee that projected gradient descent finds an $r(n_\target)$--suboptimal point.
  Therefore, by choosing $(c_1, c_2)$ in order to achieve the minimal rate $r(n_\target)$ in \lemmaref{lemma:lin-targ-stat-rates}, we can guarantee that
  \[
    \min_{t}\frac{1}{n_\target}\norm[2]{X(\theta_t - \theta^\ast)}^2 \lesssim r(n_\target).
  \]
  Finally, due to target covariance concentration as guaranteed by the event in \lemmaref{lemma:lin-targ-cov-concentration}, we thus have that the excess risk of the best predictor found by the algorithm on the target task is bounded as
  \[
    \min_t\expt{(x^\top\theta_t - x^\top\theta_t^\ast)^2} = \min_t\norm[2]{\Sigma^{1/2}(\theta_t - \theta^\ast)}^2 \lesssim \min(r_\target^{(1)}(n), r_\target^{(2)}(n), r_\target^{(3)}(n)). \qedhere
  \]
\end{proof}


==> results/linear/perf/linOptConstants.tex <==
\begin{restatable}{lemma}{linOptConstants}
  \label{lemma:lin-opt-consts}
  Let $\tilde{w}$, $\bar{w}$, and $\bar\delta$ be defined as in \lemmaref{lemma:lin-targ-stat-rates}.
  Then, assuming that the high-probability event in \lemmaref{lemma:lin-targ-cov-concentration} holds, the three quantities above are norm-bounded by $\kappa^{1/2}(\norm[2]{B^\ast w^\ast} + \delta_0)$, up to constant factors.
  Furthermore, we can also bound $\norm[2]{\bar\delta}$ as
  \[
    \norm[2]{\bar\delta} \leq \delta_0 + \left(\frac{\norm[2]{w^\ast} + \delta_0\kappa^{1/2}}{\lambda_{\min}^{1/2}}\right)\norm[F]{P_{\Sigma^{1/2}B_0}^\perp\Sigma^{1/2}B^\ast}.
  \]
\end{restatable}
\begin{proof}
  Throughout the proof, we will write $\lambda_{\max}$ and $\lambda_{\min}$ as shorthand for $\lambda_{\max}(\Sigma)$ and $\lambda_{\min}(\Sigma)$, respectively.
  By definition, since $B_0$ is assumed to be orthonormal, the concentration of the sample covariance in \lemmaref{lemma:lin-targ-cov-concentration} implies that
  \begin{align*}
    \norm[2]{\bar{w}}^2 &\lesssim \frac{1}{n_\target\lambda_{\min}}\norm[2]{XB_0\bar{w}}^2 = \frac{1}{n_\target\lambda_{\min}}\norm[2]{P_{XB_0}X\theta^\ast}^2 \lesssim \frac{1}{\lambda_{\min}}\norm[2]{\Sigma^{1/2}\theta^\ast}^2 \leq   \kappa\norm[2]{\theta^\ast}^2 \\
    &\leq \kappa(\norm[2]{B^\ast w^\ast} + \delta_0)^2.
  \end{align*}
  Following similar arguments for $\tilde{w}$ and $\bar\delta$, we obtain the same bounds.
  Thus, we have demonstated that all three quantities are indeed norm-bounded by $\kappa^{1/2}(\norm[2]{B^\ast w^\ast} + \delta_0)$, up to constant factors.

  Finally, we proceed to derive the final bound on $\bar\delta$.
  Note that $X\bar\delta = X\delta^\ast - P_{XB_0}X\delta^\ast + P_{XB_0}^\perp XB^\ast w^\ast$.
  Therefore,
  \begin{align*}
    \norm[2]{\bar\delta} &\lesssim \delta_0 + \frac{1}{\sqrt{n_\target\lambda_{\min}}}\left[\norm[2]{P_{XB_0}X\delta^\ast} + \norm[2]{P_{XB_0}^\perp XB^\ast w^\ast}\right] \\
      &\lesssim \delta_0 + \frac{1}{\lambda_{\min}^{1/2}}\left[\norm[2]{P_{\Sigma^{1/2}B_0}\Sigma^{1/2}\delta^\ast} + \norm[2]{P_{\Sigma^{1/2}B_0}^\perp \Sigma^{1/2}B^\ast w^\ast}\right] \\
      &\lesssim \delta_0 + \frac{1}{\lambda_{\min}^{1/2}}\left[\norm[2]{\Sigma^{1/2}\delta^\ast}\norm[F]{P_{\Sigma^{1/2}B_0}P_{\Sigma^{1/2}B^\ast}^\perp} + \norm[2]{w^\ast}\norm[F]{P_{\Sigma^{1/2}B_0}^\perp \Sigma^{1/2}B^\ast}\right]
  \end{align*}
  Now, by applying the properties of the trace operator and \propref{prop:mat-to-proj},
  \begin{align*}
    \norm[F]{P_{\Sigma^{1/2}B_0}P_{\Sigma^{1/2}B^\ast}^\perp}^2 &= \tr P_{\Sigma^{1/2}B_0}P_{\Sigma^{1/2}B^\ast}^\perp P_{\Sigma^{1/2}B_0} = \tr{(I - P_{\Sigma^{1/2}B^\ast})P_{\Sigma^{1/2}B_0}} \\
      &= \tr{P_{\Sigma^{1/2}B_0} - P_{\Sigma^{1/2}B^\ast}P_{\Sigma^{1/2}B_0}} \\
      &\leq \tr{P_{\Sigma^{1/2}B^\ast} - P_{\Sigma^{1/2}B^\ast}P_{\Sigma^{1/2}B_0}} = \tr{P_{\Sigma^{1/2}B^\ast}(I - P_{\Sigma^{1/2}B_0})} \\
      &= \tr{P_{\Sigma^{1/2}B^\ast}P_{\Sigma^{1/2}B_0}^\perp}P_{\Sigma^{1/2}B^\ast} = \norm[F]{P_{\Sigma^{1/2}B_0}^\perp P_{\Sigma^{1/2}B^\ast}}^2 \\
      &\leq \frac{1}{\lambda_{\min}}\norm[F]{P_{\Sigma^{1/2}B_0}^\perp\Sigma^{1/2}B^\ast}^2,
  \end{align*}
  and thus
  \begin{align*}
    \norm[2]{\bar\delta} &\lesssim \delta_0 + \frac{1}{\lambda_{\min}^{1/2}}\left[\frac{1}{\lambda_{\min}^{1/2}}\norm[2]{\Sigma^{1/2}\delta^\ast} + \norm[2]{w^\ast}\right]\norm[F]{P_{\Sigma^{1/2}B_0}^\perp \Sigma^{1/2}B^\ast} \\
      &\leq \delta_0 + \left(\frac{\norm[2]{w^\ast} + \delta_0\kappa^{1/2}}{\lambda_{\min}^{1/2}}\right)\norm[F]{P_{\Sigma^{1/2}B_0}^\perp\Sigma^{1/2}B^\ast}. \qedhere
  \end{align*}
\end{proof}


==> results/linear/perf/linSrcCovConcentration.tex <==
\begin{restatable}[Source covariance concentration, \citet{du2020few}, Claim A.1]{lemma}{linSrcCovConcentration}
  \label{lemma:lin-src-cov-concentration}
  If $n_\source \gg \rho^4[d + \log(T/\delta)]$, then with probability at least $1 - \delta/9$ over the random draw of $n_\source T$ source inputs,
  \[
    0.9\Sigma \preceq \frac{1}{n_\source}X_t^\top X_t \preceq 1.1\Sigma
  \]
  for any $t \in [T]$.
\end{restatable}


==> results/linear/perf/linSrcTrainBound.tex <==
\begin{restatable}[Source training bound]{lemma}{linSrcTrainBound}
  \label{lemma:lin-source-train-bound}
  Let $B_0$ be a minimizer of \eqnref{eqn:linear-source-procedure}, and $\set{(\Delta_t, w_t)}_{t \in [T]}$ be minimizers for the inner optimization problem given $B_0$.
  If the regularizer coefficients are chosen such that
  \[
    \lambda \asymp \frac{1}{T\delta_0}\left[\frac{\sigma\norm[2]{\Sigma}^{1/2}}{\sqrt{n_\source T}}\sqrt{kT + kd\log\kappa n_\source + \log\frac{1}{\delta}} + \frac{\sigma}{\sqrt{n_\source}}\sqrt{\tr{\Sigma}\left(1 + \log\frac{T}{\delta}\right)}\right],
  \]
  and $\gamma = \delta_0^2\lambda$,
  then with probability at least $1 - \delta/3$,
  \[
    \begin{aligned}
      &\frac{1}{T}\sum_{t \in [T]}\norm[2]{\Sigma^{1/2}(\theta_t^\ast - \hat\theta_t)}^2 \\
        &\quad \lesssim \frac{\sigma^2}{n_\source T}\left(kT + kd\log\kappa n_\source + \log\frac{1}{\delta}\right) + \frac{\sigma\delta_0\norm[2]{\Sigma}^{1/2}}{\sqrt{n_\source T}}\sqrt{kT + kd\log\kappa n_\source + \log\frac{1}{\delta}} \\
        &\quad+ \frac{\sigma\delta_0}{\sqrt{n_\source}}\sqrt{\tr{\Sigma}\left(1 + \log\frac{T}{\delta}\right)}.
    \end{aligned}
  \]
\end{restatable}
\begin{proof}
  Throughout this proof, we instantiate the high-probability event in \lemmaref{lemma:lin-src-cov-concentration}, which occurs with probability at least $1 - \delta/9$.

  Note that we can express $\delta_t^\ast$ as $[\delta_t^\ast (w_t^\ast)^\top/\norm[2]{w_t^\ast}^2]w_t^\ast = \Delta_t^\ast w_t^\ast$.
  Thus, via the optimality of $B_0$ and $\set{(\Delta_t, w_t)}_{t \in [T]}$, we can form the basic inequality
  \begin{align*}
    &\sum_{t \in [T]}\frac{1}{2n_\source T}\norm[2]{y_t - X_t\hat\theta_t}^2 + \frac{\lambda}{2}\norm[F]{\Delta_t}^2 + \frac{\gamma}{2}\norm[2]{w_t}^2 \\
      &\qquad \leq \sum_{t \in [T]}\frac{1}{2n_\source T}\norm[2]{z_t}^2 + \frac{\lambda}{2}\norm[F]{\Delta_t^\ast}^2 + \frac{\gamma}{2}\norm[2]{w_t^\ast}^2 \\
      &\qquad \leq \sum_{t \in [T]}\frac{1}{2n_\source T}\norm[2]{z_t}^2 + \frac{\lambda}{2}\sum_{t \in [T]}\frac{\norm[2]{\delta_t^\ast}^2}{\norm[2]{w_t^\ast}^2} + \frac{\gamma}{2}\sum_{t \in [T]}\norm[2]{w_t^\ast}^2 \\
      &\qquad \leq \sum_{t \in [T]}\frac{1}{2n_\source T}\norm[2]{z_t}^2 + \left(\frac{\lambda\delta_0^2 + \gamma}{2}\right)T \\
      &\qquad \leq \underbrace{\frac{\sigma\delta_0\norm[2]{\Sigma}^{1/2}}{\sqrt{nT}}\sqrt{kT + kd\log\kappa n_\source + \log\frac{1}{\delta}} + \frac{\sigma\delta_0}{\sqrt{n}}\sqrt{\tr\Sigma\left(1 + \log\frac{T}{\delta}\right)}}_{\asdef C_{n_\source, T}} \\
      &\qquad\qquad + \sum_{t \in [T]}\frac{1}{2n_\source T}\norm[2]{z_t}^2.
  \end{align*}
  Note that the simplification of the regularizer on the optimum holds since $\norm[2]{w_t^\ast} = \Theta(1)$ by \assumpref{assump:lin-diversity-cond}.
  Equivalently, by rearranging,
  \[
    \begin{aligned}
      &\sum_{t \in [T]}\frac{1}{2n_\source T}\norm[2]{X_t(\theta_t^\ast - \hat\theta_t)}^2 + \frac{\lambda}{2}\norm[F]{\Delta_t}^2 + \frac{\gamma}{2}\norm[2]{w_t}^2 \\
        &\quad \leq \sum_{t \in [T]}\frac{1}{2n_\source T}\inprod{z_t, X_t(\theta_t^\ast - \hat\theta_t)} + C_{n_\source, T}.
    \end{aligned}
  \]
  Finally, by \propref{prop:sum-regularizers-equivalence}, the regularizer on $\Delta_t$ and $w_t$ can be rewritten as a regularizer on $\hat\delta_t$, i.e.
  \begin{equation}
    \label{eqn-int:lin-src-basic-ineq}
    \sum_{t \in [T]}\frac{1}{2n_\source T}\norm[2]{X_t(\theta_t^\ast - \hat\theta_t)}^2 + \sqrt{\lambda\gamma}\norm[2]{\hat\delta_t} \leq \sum_{t \in [T]}\frac{1}{2n_\source T}\inprod{z_t, X_t(\theta_t^\ast - \hat\theta_t)} + C_{n_\source, T}.
  \end{equation}

  To proceed, define the set $S$ as
  \[
    \set{[\alpha_t + \beta_t]_{t \in [T]} \suchthat \rank{[\alpha_t]} \leq 2k, \norm[2]{\beta_t} \leq \delta_0 + \norm[2]{\hat\delta_t}, \norm[2]{X_t(\alpha_t + \beta_t)} \leq \norm[2]{X_t(\theta_t^\ast - \hat\theta_t)}},
  \]
  and observe that $[\theta_t^\ast - \hat\theta_t]_{t \in [T]} \in S$, by letting $\alpha_t = B^\ast w_t^\ast - B_0w_t$ and $\beta_t = \delta_t^\ast - \hat\delta_t$.
  We bound the right-hand side of \eqnref{eqn-int:lin-src-basic-ineq} via bounding the supremum of the inner product over $S$, i.e.
  \[
     \sum_{t \in [T]}\inprod{z_t, X_t(\theta_t^\ast - \hat\theta_t)} \leq \sup_{[\alpha_t + \beta_t] \in S}\sum_{t \in [T]}\inprod{z_t, X_t(\alpha_t + \beta_t)}.
  \]
  Now, we decompose the Gaussian width as
  \[
    \sup_{[\alpha_t + \beta_t] \in S}\sum_{t \in [T]}\inprod{z_t, X_t(\alpha_t + \beta_t)} \leq \underbrace{\sup_{[\alpha_t] \in S}\sum_{t \in [T]}\inprod{z_t, X_t\alpha_t}}_{\text{(I)}} + \underbrace{\sup_{[\beta_t] \in S_2}\sum_{t \in [T]}\inprod{z_t, X_t\beta_t}}_{\text{(II)}},
  \]
  where $S_2 = \set{[\beta_t]_{t \in [T]} \suchthat \norm[2]{\beta_t} \leq \delta_0 + \norm[2]{\hat\delta_t}}$.
  Note the abuse of notation in (I), where we say $[\alpha_t]_{t \in [T]} \in S$ if there exists $[\beta_t]_{t \in [T]}$ so that $[\alpha_t + \beta_t]_{t \in [T]} \in S$.
  This decomposes the Gaussian width into the sum of the Gaussian widths of a low-rank set (I) and a small norm set (II).
  We proceed to bound both terms accordingly to these two properties.

  \vspace{2ex}
  \noindent
  \underline{Bounding the Gaussian width of the low-rank set (I)}.
  \vspace{1ex}

  To bound the Gaussian width, we first enlarge $S$ to remove $\beta_t$ from the definition of the feasible set.
  Fix any $(\alpha_t, \beta_t)$ pair satisfying the conditions in $S$, and note that
  \[
    \norm[2]{X_t\beta_t} \lesssim \sqrt{n_\source}\norm[2]{\Sigma}^{1/2}\left(\delta_0 + \norm[2]{\hat\delta_t}\right).
  \]
  Therefore, by the reverse triangle inequality,
  \begin{align*}
    &\abs{\norm[2]{X_t\alpha_t} - \norm[2]{X_t\beta_t}} \leq \norm[2]{X_t(\alpha_t + \beta_t)} \\
      &\qquad \implies \norm[2]{X_t\alpha_t} \leq \underbrace{\norm[2]{X_t(\theta_t^\ast - \hat\theta_t)} + \sqrt{n_\source}\norm[2]{\Sigma}^{1/2}\left(\delta_0 + \norm[2]{\hat\delta_t}\right)}_{\asdef \rho_t}.
  \end{align*}
  Consequently, we can enlarge the feasible set to
  \[
    S_1 \defas \set{[\alpha_t] \suchthat \rank{[\alpha_t]} \leq 2k, \norm[2]{X_t\alpha_t} \leq \rho_t}.
  \]
  Having relaxed the constraints, we now proceed to the main argument.

  Since $\rank{[\alpha_t]} \leq 2k$, there exists an orthogonal matrix $V \in \reals^{d \times 2k}$ (dependent on $\alpha_t$) and vectors $r_t \in \reals^{2k}$ such that $\alpha_t = Vr_t$.
  Therefore, the inner product in the Gaussian width would be unchanged if we project $z_t$ onto $X_tV$, i.e.
  \[
    \sup_{[\alpha_t] \in S_1}\sum_{t \in [T]}\inprod{z_t, X_t\alpha_t} = \sup_{[\alpha_t] \in S_1}\sum_{t \in [T]}\inprod{P_{X_tV}z_t, X_tVr_t}.
  \]
  The key idea we will leverage is that if $V$ were chosen independently of $z_t$, then $P_{X_tV}z_t$ is Gaussian in a $2k$-dimensional space, and thus norm bounded by $\tilde{O}(\sqrt{2k})$ with high probability.
  However, due to the supremum over $\alpha_t$, this independence assumption is not satisfied.
  Nevertheless, we can obtain a \emph{fixed} finite covering of the set of all rank-$2k$ matrices, and ensure that the aforementioned norm bound on $P_{X_tV}z_t$ holds for every $V$ in the covering via a union-bound.
  By choosing the discretization level of the covering appropriately, we can control the error resulting from approximating the supremum by some element of the covering.

  Formally, let $\orthogonal^{d \times 2k}$ be the set of orthogonal matrices in $\reals^{d \times 2k}$.
  By \propref{prop:orth-mat-covering}, there exists an $\epsilon$-covering of $\orthogonal^{d \times 2k}$ in the Frobenius norm with at most $(6\sqrt{2k}/\epsilon)^{2kd}$ elements.
  Let $\bar{V}$ be an element of the covering such that $\norm[F]{V - \bar{V}} \leq \epsilon$.
  Then,
  \begin{align*}
    \inprod{z_t, X_t\alpha_t} &= \inprod{z_t, X_t\bar{V}r_t} + \inprod{z_t, X_t(V - \bar{V})r_t} \\
      &\leq \norm[2]{P_{X_t\bar{V}}z_t}\norm[2]{X_t\bar{V}r_t} + \norm[2]{z_t}\norm[2]{X_t(V - \bar{V})r_t} \\
      &\leq \norm[2]{P_{X_t\bar{V}}z_t}\norm[2]{X_tVr_t} + (\norm[2]{P_{X_t\bar{V}}z_t} + \norm[2]{z_t})\norm[2]{X_t(V - \bar{V})r_t} \\
      &\leq \norm[2]{P_{X_t\bar{V}}z_t}\norm[2]{X_tVr_t} + (\norm[2]{P_{X_t\bar{V}}z_t} + \norm[2]{z_t})\norm[2]{X_t(V - \bar{V})r_t} \\
      &\lesssim \norm[2]{P_{X_t\bar{V}}z_t}\norm[2]{X_t\alpha_t} + \norm[2]{z_t}\norm[2]{X_t(V - \bar{V})r_t},
  \end{align*}
  and thus
  \begin{align*}
    \sum_{t \in [T]}\inprod{z_t, X_tVr_t} &\leq \sqrt{\smash[b]{\underbrace{\left(\sum_{t \in [T]}\norm[2]{P_{X_t\bar{V}}z_t}^2\right)}_{(\text{A})}}\left(\sum_{t \in [T]}\norm[2]{X_t\alpha_t}^2\right)}\vphantom{\underbrace{\left(\sum_{t \in [T]}\right)}_{(A)}} \\
      &\quad + \sqrt{\smash[b]{\underbrace{\left(\sum_{t \in [T]}\norm[2]{z_t}^2\right)}_{(\text{B})}}\smash[b]{\underbrace{\left(\sum_{t \in [T]}\norm[2]{X_t(V - \bar{V})r_t}\right)}_{(\text{C})}}\vphantom{\left(\sum_{t \in [T]}\right)}}.\vphantom{\underbrace{\left(\sum_{t \in [T]}\right)}_{(A)}}
  \end{align*}
  We will bound (A), (B), and (C) individually.

  \begin{enumerate}[label=(\Alph*)]
    \item For a fixed $\bar{V}$, (A) is a chi-squared random variable with $kT$ degrees of freedom scaled by $\sigma^2$.
      However, since $\bar{V}$ depends on $V$, we need to have a high probability bound for any element of the covering.
      By using known concentration bounds for chi-squared random variables together with the union-bound, we find that uniformly over the covering,
      \[
        (\mathrm{A}) \leq \sigma^2\left(kT + \log\frac{1}{\delta'}\right) \qquad \text{w.p. $\geq 1 - \delta'\left(\frac{6\sqrt{2k}}{\epsilon}\right)^{2kd}$}.
      \]

    \item Note that (B) is a chi-squared random variable with $n_\source T$ degrees of freedom scaled by $\sigma^2$, and thus
  \[
    (\mathrm{B}) \lesssim \sigma^2\left(n_\source T + \log\frac{1}{\delta}\right) \qquad \text{w.p. $\geq 1 - \frac{\delta}{18}$}.
  \]

    \item Since $(1/n_\source)X^\top X$ is concentrated about $\Sigma$ via \lemmaref{lemma:lin-src-cov-concentration},
      \begin{align*}
        \norm[2]{X_t(V - \bar{V})r_t}^2 &\lesssim n_\source\norm[2]{\Sigma}\epsilon^2\norm[2]{r_t}^2 = n_\source\norm[2]{\Sigma}\epsilon^2\norm[2]{Vr_t}^2 \lesssim \kappa\epsilon^2\norm[2]{X_tVr_t}^2.
      \end{align*}
  \end{enumerate}

  Putting these bounds together, and setting $\epsilon = \sqrt{k/\kappa n_\source}$ and $\delta' = \delta/[18(6\sqrt{2k}/\epsilon)^{2kd}]$, we obtain
  \begin{align*}
      \sum_{t \in [T]}\inprod{z_t, X_t\alpha_t} &\lesssim \left(\sigma\sqrt{kT + \log\frac{1}{\delta'}} + \epsilon\sigma\sqrt{\kappa n_\source T + \log\frac{1}{\delta}}\right)\sqrt{\left(\sum_{t \in [T]}\norm[2]{X_tVr_t}^2\right)} \\
        &\lesssim \left(\sigma\sqrt{kT + \log\frac{1}{\delta'}}\right)\sqrt{\left(\sum_{t \in [T]}\norm[2]{X_tVr_t}^2\right)} \qquad\qquad (k < n_\source, \delta' < \delta) \\
        &\lesssim \sigma\sqrt{kT + kd\log\kappa n_\source + \log\frac{1}{\delta}}\sqrt{\left(\sum_{t \in [T]}\norm[2]{X_t\alpha_t}^2\right)}.
  \end{align*}
  Taking the supremum over $S_1$, we thus obtain the following bound on the Gaussian width:
  \begin{align*}
    &\sup_{[\alpha_t] \in S_1}\sum_{t \in [T]}\inprod{z_t, X_t\alpha_t} \\
      &\quad\lesssim \sigma\sqrt{kT + kd\log\kappa n_\source + \log\frac{1}{\delta}}\left[\sqrt{\sum_{t \in [T]}\norm[2]{X_t(\theta_t^\ast - \hat\theta_t)}^2\vphantom{\sum^T}} + \sqrt{\norm[2]{\Sigma}n_\source T}\left(\delta_0 + \norm[2]{\hat\delta_t}\right)\right].
  \end{align*}
  Note that the events for this sub-argument occur with probability at least $1 - \delta/9$.

  \clearpage

  \vspace{2ex}
  \noindent
  \underline{Bounding the Gaussian width of the low-norm set (II)}.
  \vspace{1ex}

  Recall that we want to bound
  \[
    \sup_{[\beta_t] \in S_2}\sum_{t \in [T]}\inprod{z_t, X_t\beta_t}, \quad S_2 \defas \set{[\beta_t] \suchthat \norm[2]{\beta_t} \leq \delta_0 + \norm[2]{\hat\delta_t}}.
  \]
  For any $t \in [T]$,
  \[
    \inprod{z_t, X_t\beta_t} = \inprod{X_t^\top z_t, \beta_t} \leq \left(\delta_0 + \norm[2]{\hat\delta_t} \right)\norm[2]{X_t^\top z_t}.
  \]
  Furthermore, by the Hanson-Wright inequality, we have that with probability at least $1 - \delta/9T$,
  \[
    \norm[2]{X_t^\top z_t} \lesssim \sigma\sqrt{n_\source\tr\Sigma\left(1 + \log\frac{T}{\delta}\right)}.
  \]
  Putting everything together, we thus find that with probability at least $1 - \delta/9$,
  \[
    \sup_{[\beta_t] \in S_2}\sum_{t \in [T]}\inprod{z_t, X_t\beta_t} \leq \sigma \left(T\delta_0 + \sum_{t \in [T]}\norm[2]{\hat\delta_t}\right)\sqrt{n_\source\tr\Sigma\left(1 + \log\frac{T}{\delta}\right)}.
  \]

  \vspace{2ex}
  \noindent
  \underline{Combining the bounds and concluding}.
  \vspace{1ex}

  Having bounded both Gaussian widths, we can thus bound the right-hand side of \eqnref{eqn-int:lin-src-basic-ineq} as
  \begin{equation*}
    \begin{aligned}
      &\sum_{t \in [T]}\frac{1}{2n_\source T}\norm[2]{X_t(\theta_t^\ast - \hat\theta_t)}^2 + \left(\sqrt{\lambda\gamma} - \frac{1}{\delta_0T}C_{n_\source, T}\right)\norm[2]{\hat\delta_t} \\
        &\quad \lesssim \frac{\sigma}{\sqrt{nT}}\sqrt{kT + kd\log\kappa n_\source + \log\frac{1}{\delta}}\left(\sum_{t \in [T]}\frac{1}{2n_\source T}\norm[2]{X_t(\theta_t^\ast - \hat\theta_t)}^2\right)^{1/2} + C_{n_\source, T}.
    \end{aligned}
  \end{equation*}
  Therefore, as long as $\sqrt{\lambda\gamma} \geq (1/\delta_0T)C_{n_\source, T}$,
  \begin{align*}
      &\sum_{t \in [T]}\frac{1}{2n_\source T}\norm[2]{X_t(\theta_t^\ast - \hat\theta_t)}^2 \\
        &\quad \lesssim \frac{\sigma}{\sqrt{n_\source T}}\sqrt{kT + kd\log\kappa n_\source + \log\frac{1}{\delta}}\left(\sum_{t \in [T]}\frac{1}{2n_\source T}\norm[2]{X_t(\theta_t^\ast - \hat\theta_t)}^2\right)^{1/2} + C_{n_\source, T}.
  \end{align*}
  Finally, by solving the quadratic inequality using \propref{prop:solve-quad-ineqs}, we find that
  \begin{align*}
    &\sum_{t \in [T]}\frac{1}{2n_\source T}\norm[2]{X_t(\theta_t^\ast - \hat\theta_t)}^2 \\
      &\quad \lesssim \frac{\sigma^2}{n_\source T}\left(kT + kd\log\kappa n_\source + \log\frac{1}{\delta}\right) + \frac{\sigma\delta_0\norm[2]{\Sigma}^{1/2}}{\sqrt{n_\source T}}\sqrt{kT + kd\log\kappa n_\source + \log\frac{1}{\delta}} \\
      &\qquad\qquad + \frac{\sigma\delta_0}{\sqrt{n_\source}}\sqrt{\tr{\Sigma}\left(1 + \log\frac{T}{\delta}\right)},
  \end{align*}
  from which the desired performance bound follows due to the concentration of the empirical covariance from \lemmaref{lemma:lin-src-cov-concentration}.
  Since the concentration of the source covariance matrices and each of the sub-arguments all hold with probability at least $1 - \delta/9$, it follows that the main claim holds with probability at least $1 - \delta/3$.
\end{proof}


==> results/linear/perf/linTargCovConcentration.tex <==
\begin{restatable}[Target covariance concentration]{lemma}{linTargCovConcentration}
  \label{lemma:lin-targ-cov-concentration}
  If $n_\target \gg \rho^4[d + \log(T/\delta)]$, then with probability at least $1 - \delta/9$ over the random draw of $n_\target$ target inputs,
  \[
    0.9\Sigma \preceq \frac{1}{n_\target}X^\top X \preceq 1.1\Sigma
  \]
  for any $t \in [T]$.
\end{restatable}
\begin{proof}
  The proof is similar to that of \lemmaref{lemma:lin-src-cov-concentration}, and is omitted for brevity.
\end{proof}


==> results/linear/perf/linTargStatRates.tex <==
\begin{restatable}[Statistical Rates for $\meanloss_\beta$]{lemma}{linTargStatRates}
  \label{lemma:lin-targ-stat-rates}
  Assume that $(\Delta, w)$ is $\zeta$-suboptimal for $\meanloss_\beta$ with the constraint set $\constraintset_\beta = \set{(\Delta, w) \suchthat \norm[F]{\Delta} \leq c_1/\beta, \norm[2]{w} \leq c_2/\beta}$, i.e.
  \[
    \meanloss_\beta(\Delta, w) \leq \min_{(\Delta', w') \in \constraintset_\beta}\meanloss_\beta(\Delta', w') + \zeta.
  \]
  We write $\hat\theta$ for the predictor corresponding to $(\Delta, w)$, i.e. $\hat\theta = \beta(A_{B_0} + \Delta)(w_0 + w)$.
  Now, let
  \begin{align*}
    \bar{w} &= (B_0X^\top XB_0)^\dagger B_0^\top X^\top X\theta^\ast \\
    \bar\delta &= \theta^\ast - B_0\bar{w} \\
    \tilde{w} &= (B_0^\top X^\top XB_0)^\dagger B_0^\top X^\top XB^\ast w^\ast.
  \end{align*}
  Note that $XB_0\bar{w} = P_{XB_0}X\theta^\ast$, $X\bar\delta = P_{XB_0}^\perp X\theta^\ast$, and $XB\tilde{w} = P_{XB_0}XB^\ast w^\ast$.
  Then, assuming $\beta > \max(\norm[2]{\bar{w}}, \norm[2]{\tilde{w}})$,
  \[
    \frac{1}{2n_\target}\norm[2]{X(\theta^\ast - \hat\theta)}^2 \lesssim \zeta +
    \begin{cases}
      \!\begin{aligned}
        &\norm[2]{P_{\Sigma^{1/2}B_0}^\perp \Sigma^{1/2}B^\ast w^\ast}^2 \\
        &\qquad + \frac{\sigma^2}{n_\target}\left(k + \log\frac{1}{\delta}\right) \\
        &\qquad + \frac{\sigma\delta_0}{\sqrt{n_\target}}\sqrt{\tr\Sigma\left(1 + \log\frac{1}{\delta}\right)}
      \end{aligned} & c_1 = \delta_0, c_2 = \norm[2]{\tilde{w}} \\[9ex]
      \!\begin{aligned}
        &\frac{\sigma^2}{n_\target}\left(k + \log\frac{1}{\delta}\right) \\
        &\qquad + \frac{\sigma\norm[2]{\bar\delta}}{\sqrt{n_\target}}\sqrt{\tr\Sigma\left(1 + \log\frac{1}{\delta}\right)}
      \end{aligned} & c_1 = \norm[2]{\bar\delta}, c_2 = \norm[2]{\bar{w}} \\[7ex]
      \displaystyle \frac{\sigma^2}{n_\target}\left(d + \log\frac{1}{\delta}\right) & c_1 = \norm[2]{\theta^\ast}, c_2 = 0
    \end{cases}
  \]
  with probability at least $1 - \delta/3$.
\end{restatable}
\begin{proof}
  We proceed by proving the three cases separately.
  Throughout the proof, we instantiate the high-probability event in \lemmaref{lemma:lin-targ-cov-concentration}, which guarantees that
  \[
    0.9\Sigma \preceq \frac{1}{n_\target}X^\top X \preceq 1.1\Sigma.
  \]
  Recall that this event occurs with probability at least $1 - \delta/9$.

  \vspace{2ex}
  \noindent
  \underline{$c_1 = \delta_0, c_2 = \norm[2]{\tilde{w}}$}
  \vspace{1ex}

  Due to the choice of $c_1$ and $c_2$, there exists a parameter in $\constraintset_\beta$ corresponding to the prediction vector $P_{XB_0}X\theta^\ast + X\delta^\ast$.
  Writing the corresponding basic inequality, we thus have that
  \begin{align*}
    &\frac{1}{2n_\target}\norm[2]{y - X\hat\theta}^2 - \zeta \leq \frac{1}{2n_\target}\norm[2]{P_{XB_0}^\perp XB^\ast w^\ast}^2 + \frac{1}{n_\target}\inprod{z, P_{XB_0}^\perp XB^\ast w^\ast} + \frac{1}{2n_\target}\norm[2]{z}^2 \\[1ex]
    &\qquad \implies \frac{1}{2n_\target}\norm[2]{X(\theta^\ast - \hat\theta)}^2 \leq \zeta + \frac{1}{2n_\target}\norm[2]{P_{XB_0}^\perp XB^\ast w^\ast}^2 + \frac{1}{n_\target}\inprod{z, P_{XB_0}^\perp XB^\ast w^\ast} \\
    &\qquad\qquad\qquad\qquad\qquad\qquad\qquad - \frac{1}{n_\target}\inprod{z, X(\theta^\ast - \hat\theta)}.
  \end{align*}
  Simplifying further,
  \begin{align*}
    &\frac{1}{n_\target}\inprod{z, P_{XB_0}^\perp XB^\ast w^\ast} - \frac{1}{n_\target}\inprod{z, X(\theta^\ast - \hat\theta)} \\
      &\qquad = \frac{1}{n_\target}\inprod{z, P_{XB_0}X(\hat\theta - \theta^\ast)} - \frac{1}{n_\target}\inprod{z, P_{XB_0}^\perp X(\delta^\ast - \beta\Delta(w_0 + w))}.
  \end{align*}
  Now, by the Hanson-Wright inequality, we can bound the last term as
  \begin{align*}
    -\frac{1}{n_\target}\inprod{X^\top P_{XB_0}^\perp z, \delta^\ast - \beta\Delta(w_0 + w)} &\leq \frac{1}{n_\target}\norm[2]{X^\top P_{XB_0}^\perp z}\norm[2]{\delta^\ast + \beta\Delta(w_0 + w)} \\
      &\lesssim \frac{\sigma\delta_0}{\sqrt{n_\target}}\sqrt{\tr\Sigma\left(1 + \log\frac{1}{\delta}\right)}
  \end{align*}
  with probability at least $1 - \delta/9$.
  Therefore, we can rewrite the prior basic inequality as
  \begin{align*}
    \frac{1}{2n_\target}\norm[2]{X(\theta^\ast - \hat\theta)}^2 &\lesssim \underbrace{\frac{1}{2n_\target}\norm[2]{P_{XB_0}^\perp XB^\ast w^\ast}^2 + \frac{\sigma\delta_0}{\sqrt{n_\target}}\sqrt{\tr\Sigma\left(1 + \log\frac{1}{\delta}\right)} + \zeta}_{\asdef C} \\
      &\qquad + \frac{1}{n_\target}\inprod{z, P_{XB_0}X(\theta^\ast - \hat\theta)}.
  \end{align*}
  Now, note that we can form the quadratic inequality
  \[
    \frac{1}{n_\target}\norm[2]{P_{XB_0}X(\theta^\ast - \hat\theta)}^2 \leq \frac{1}{n_\target}\norm[2]{P_{XB_0}z}\norm[2]{P_{XB_0}X(\theta^\ast - \hat\theta)} + C,
  \]
  and thus by applying \propref{prop:solve-quad-ineqs} to solve the inequality and noting that $P_{XB_0}z/\sigma$ is distributed as a chi-squared random variable with $k$ degrees of freedom,
  \begin{align*}
    \frac{1}{n_\target}\norm[2]{X(\theta^\ast - \hat\theta)}^2 &\lesssim \zeta + \norm[2]{P_{\Sigma^{1/2}B_0}^\perp \Sigma^{1/2}B^\ast w^\ast}^2 \\
      &\qquad + \frac{\sigma^2}{n_\target}\left(k + \log\frac{1}{\delta}\right) + \frac{\sigma\delta_0}{\sqrt{n_\target}}\sqrt{\tr\Sigma\left(1 + \log\frac{1}{\delta}\right)}
  \end{align*}
  with probability at least $1 - \delta/9$, which is the bound that we wanted to show.

  \vspace{2ex}
  \noindent
  \underline{$c_1 = \norm[2]{\bar\delta}, c_2 = \norm[2]{\bar{w}}$}
  \vspace{1ex}

  Due to the choice of $c_1$ and $c_2$, there exists a parameter in $\constraintset_\beta$ corresponding to a predictor that agrees with $\theta^\ast$ on the target samples.
  Therefore,
  \begin{align}
    &\frac{1}{2n_\target}\norm[2]{X(\theta^\ast - \hat\theta)}^2 \leq \zeta + \frac{1}{2n_\target}\norm[2]{z}^2 \nonumber \\[1ex]
    &\qquad \implies \frac{1}{2n_\target}\norm[2]{X(\theta^\ast - \hat\theta)}^2 \leq \zeta + \frac{1}{n_\target}\inprod{z, P_{XB_0}X(\theta^\ast - \hat\theta)} + \frac{1}{n_\target}\inprod{z, P_{XB_0}^\perp X(\theta^\ast - \hat\theta)}. \label{eqn-int:lin-targ-basic-ineq}
  \end{align}
  We proceed with an argument similar to that used in the source guarantee, albeit simpler since the representation $B_0$ is fixed (and thus no covering argument is required).
  Along these lines, we bound the first term using the low-rank of $B_0$.
  Via projections,
  \begin{align*}
    &\frac{1}{n_\target}\norm[2]{P_{XB_0}X(\theta^\ast - \hat\theta)}^2 \\ &\qquad \lesssim \zeta + \frac{1}{n_\target}\norm[2]{P_{XB_0}z}\norm[2]{P_{XB_0}X(\theta^\ast - \hat\theta)} + \frac{1}{n_\target}\inprod{z, P_{XB_0}^\perp X(\theta^\ast - \hat\theta)}.
  \end{align*}
  Therefore, by applying \propref{prop:solve-quad-ineqs} to solve the quadratic inequality, we have that with probability at least $1 - \delta/9$,
  \[
    \frac{1}{2n_\target}\norm[2]{X(\theta^\ast - \hat\theta)}^2 \leq \zeta + \frac{\sigma^2}{n_\target}\left(k + \log\frac{1}{\delta}\right) + \frac{1}{n_\target}\inprod{z, P_{XB_0}^\perp X(\theta^\ast - \hat\theta)}.
  \]
  To bound the second term, we simply make use of the norm constraints defining the feasible set $\constraintset_\beta$, which we note is analogous to the low-norm sub-argument of the source guarantee.
  Formally, the Hanson-Wright inequality implies that with probability at least $1 - \delta/9$,
  \begin{align*}
    \frac{1}{n_\target}\inprod{z, P_{XB_0}^\perp X(\theta^\ast - \hat\theta)} &= \frac{1}{\sqrt{n_\target}}\norm[2]{\frac{1}{\sqrt{n_\target}}X^\top P_{XB_0}^\perp z}\norm[2]{\bar\delta + \beta\Delta w_0 + \beta\Delta w} \\
      &\lesssim \frac{\sigma\norm[2]{\bar\delta}}{\sqrt{n_\target}}\sqrt{\tr\Sigma\left(1 + \log\frac{1}{\delta}\right)}.
  \end{align*}
  Putting everything together, we thus have that
  \[
    \frac{1}{2n_\target}\norm[2]{X(\theta^\ast - \hat\theta)}^2 \lesssim \zeta + \frac{\sigma^2}{n_\target}\left(k + \log\frac{1}{\delta}\right) + \frac{\sigma\norm[2]{\bar\delta}}{\sqrt{n_\target}}\sqrt{\tr\Sigma\left(1 + \log\frac{1}{\delta}\right)}.
  \]

  \vspace{2ex}
  \noindent
  \underline{$c_1 = \norm[2]{\theta^\ast}, c_2 = 0$}
  \vspace{1ex}

  Due to the choice of $c_1$ and $c_2$, there exists a parameter in $\constraintset_\beta$ corresponding to a predictor that agrees with $\theta^\ast$ on the target samples.
  Therefore, we can write the basic inequality
  \[
    \frac{1}{n_\target}\norm[2]{y - X\hat\theta}^2 \leq \zeta + \frac{1}{n_\target}\norm[2]{z}^2 \implies \frac{1}{n_\target}\norm[2]{X(\theta^\ast - \hat\theta)}^2 \leq \zeta + \frac{1}{n_\target}\inprod{z, X(\theta^\ast - \theta)}.
  \]
  Now, noting that $P_{X}z/\sigma$ is a chi-squared random variable with $d$ degrees of freedom, we have that with probability at least $1 - 2\delta/9$,
  \[
    \frac{1}{n_\target}\inprod{z, X(\theta^\ast - \hat\theta)} \leq \frac{1}{n_\target}\norm[2]{P_{X}z}\norm[2]{X(\theta^\ast - \hat\theta)} \leq \frac{1}{n_\target}\sqrt{d + \log\frac{1}{\delta}}\norm[2]{X(\theta^\ast - \hat\theta)}.
  \]
  Therefore, by solving the resulting quadratic inequality via \propref{prop:solve-quad-ineqs}, we obtain the bound
  \[
    \frac{1}{n_\target}\norm[2]{X(\theta^\ast - \hat\theta)}^2 \leq \zeta + \frac{\sigma^2}{n_\target}\left(d + \log\frac{1}{\delta}\right).
  \]

  Observe that all relevant high-probability events for each case occur simultaneously with probability at least $1 - \delta/3$, as desired.
\end{proof}


==> results/linear/perf/linTransferLemma.tex <==
\begin{restatable}[Transfer Lemma]{lemma}{linTransferLemma}
  \label{lemma:lin-transfer-lemma}
  Under \assumpref{assump:lin-diversity-cond}, we have that
  \[
    \norm[F]{P_{\Sigma^{1/2}B_0}\Sigma^{1/2}B^\ast}^2 \lesssim k\left[\frac{1}{T}\sum_{t \in [T]}\norm[2]{\Sigma^{1/2}(\theta_t^\ast - \hat\theta_t)}^2\right].
  \]
\end{restatable}
\begin{proof}
  Throughout this proof, we will write $P \defas P_{\Sigma^{1/2}B_0}$ and $P^\perp \defas P_{\Sigma^{1/2}B_0}^\perp$ for readability.
  To proceed, note that we intuitively expect that for a learner that has learned the correct spaces, $P\Sigma^{1/2}\hat\theta_t \approx \Sigma^{1/2}B^\ast w_t^\ast$ as it is the low-rank component of the estimator, and consequently, $P^\perp\Sigma^{1/2}\hat\theta_t \approx \Sigma^{1/2}\delta_t^\ast$.
  Then, decomposing into the corresponding errors, we have that for any $t \in [T]$,
  \begin{align*}
    \norm[2]{\Sigma^{1/2}(\theta_t^\ast - \hat\theta_t)}^2 &\gtrsim \norm[2]{\Sigma^{1/2}B^\ast w_t^\ast - P\Sigma^{1/2}\hat\theta_t}^2 + \norm[2]{\Sigma^{1/2}\delta_t^\ast - P^\perp \Sigma^{1/2}\hat\theta_t}^2 \\
      &\qquad + 2\inprod{\Sigma^{1/2}B^\ast w_t^\ast - P\Sigma^{1/2}\hat\theta_t, \Sigma^{1/2}\delta_t^\ast - P^\perp \Sigma^{1/2}\hat\theta_t} \\
      &\geq \norm[2]{P^\perp\Sigma^{1/2}B^\ast w_t^\ast}^2 + \norm[2]{\Sigma^{1/2}\delta_t^\ast - P^\perp \Sigma^{1/2}\hat\theta_t}^2 \\
      &\qquad - 2\abs{\inprod{\Sigma^{1/2}B^\ast w_t^\ast - P\Sigma^{1/2}\hat\theta_t, \Sigma^{1/2}\delta_t^\ast - P^\perp \Sigma^{1/2}\hat\theta_t}}.
  \end{align*}

  We proceed to bound the inner product above.
  We do so by observing that if we were to replace $\hat\theta_t$ by $\theta_t^\ast$, then
  \begin{align*}
    &\inprod{\Sigma^{1/2}B^\ast w_t^\ast - P\Sigma^{1/2}\theta_t^\ast, \Sigma^{1/2}\delta_t^\ast - P^\perp\Sigma^{1/2}\delta_t^\ast} \\
      &\qquad = \inprod{P^\perp\Sigma^{1/2}B^\ast w_t^\ast - P\Sigma^{1/2}\delta_t^\ast, P^\perp\Sigma^{1/2}\delta_t^\ast - P\Sigma^{1/2}B^\ast w_t^\ast} \\
      &\qquad = (w_t^\ast)^\top(B^\ast)^\top\Sigma\delta_t^\ast \\
      &\qquad = 0.
  \end{align*}
  To translate this result into a bound on the original inner product, we note that as $n_\source \to \infty$, and the impact of the noise and the regularizer on the optimization is diminished, we expect $\hat\theta_t$ to learn the projections of $X_t\theta_t^\ast$ onto $X_tB_0$ and its complement.
  With these two insights in mind, we decompose the inner product as
  \begin{align*}
    &\abs{\inprod{\Sigma^{1/2}B^\ast w_t^\ast - P\Sigma^{1/2}\hat\theta_t, \Sigma^{1/2}\delta_t^\ast - P^\perp \Sigma^{1/2}\hat\theta_t}} \\
      &\quad \leq \abs{\inprod{\Sigma^{1/2}B^\ast w_t^\ast - P\Sigma^{1/2}\theta_t^\ast, P^\perp \Sigma^{1/2}(\theta_t^\ast - \hat\theta_t)}} \\
      &\qquad\quad + \abs{\inprod{P\Sigma^{1/2}(\theta_t^\ast - \hat\theta_t), \Sigma^{1/2}\delta_t^\ast - P^\perp \Sigma^{1/2}\hat\theta_t}} \\[1ex]
      &\qquad\quad + \underbrace{\abs{\inprod{\Sigma^{1/2}B^\ast w_t^\ast - P\Sigma^{1/2}\theta_t^\ast, \Sigma^{1/2}\delta_t^\ast - P^\perp \Sigma^{1/2}\theta_t^\ast}}}_{= 0} \\
      &\quad = \abs{\inprod{P^\perp \Sigma^{1/2}B^\ast w_t^\ast, P^\perp \Sigma^{1/2}(\theta_t^\ast - \hat\theta_t)}} + \abs{\inprod{P\Sigma^{1/2}(\theta_t^\ast - \hat\theta_t), \Sigma^{1/2}\delta_t^\ast - P^\perp \Sigma^{1/2}\hat\theta_t}}.
  \end{align*}
  Putting everything together, we find that
  \begin{align*}
    &\frac{1}{T}\sum_{t \in [T]}\norm[2]{P^\perp\Sigma^{1/2}B^\ast w_t^\ast}^2 + \frac{1}{T}\sum_{t \in [T]}\norm[2]{\Sigma^{1/2}\delta_t^\ast - P^\perp \Sigma^{1/2}\hat\theta_t}^2 \\
    &\qquad \lesssim \frac{1}{T}\sum_{t \in [T]}\norm[2]{\Sigma^{1/2}(\theta_t^\ast - \hat\theta_t)}^2 + \frac{1}{T}\sum_{t \in [T]}\abs{\inprod{\Sigma^{1/2}B^\ast w_t^\ast - P\Sigma^{1/2}\hat\theta_t, \Sigma^{1/2}\delta_t^\ast - P^\perp \Sigma^{1/2}\hat\theta_t}} \\
    &\qquad \leq \frac{1}{T}\sum_{t \in [T]}\norm[2]{\Sigma^{1/2}(\theta_t^\ast - \hat\theta_t)}^2 + \frac{1}{T}\sum_{t \in [T]}\abs{\inprod{P^\perp \Sigma^{1/2}B^\ast w_t^\ast, P^\perp \Sigma^{1/2}(\theta_t^\ast - \hat\theta_t)}} \\
    &\qquad\qquad  + \frac{1}{T}\sum_{t \in [T]}\abs{\inprod{P\Sigma^{1/2}(\theta_t^\ast - \hat\theta_t), \Sigma^{1/2}\delta_t^\ast - P^\perp \Sigma^{1/2}\hat\theta_t}} \\
    &\qquad \leq \frac{1}{T}\sum_{t \in [T]}\norm[2]{\Sigma^{1/2}(\theta_t^\ast - \hat\theta_t)}^2 + \sqrt{\frac{1}{T}\sum_{t \in [T]}\norm[2]{P^\perp \Sigma^{1/2}(\theta_t^\ast - \hat\theta_t)}^2\vphantom{\sum^T}}\sqrt{\frac{1}{T}\sum_{t \in [T]}\norm[2]{P^\perp \Sigma^{1/2}B^\ast w_t^\ast}^2\vphantom{\sum^T}} \\
    &\qquad\qquad + \sqrt{\frac{1}{T}\sum_{t \in [T]}\norm[2]{P\Sigma^{1/2}(\theta_t^\ast - \hat\theta_t)}^2\vphantom{\sum^T}}\sqrt{\frac{1}{T}\sum_{t \in [T]}\norm[2]{\Sigma^{1/2}\delta_t^\ast - P^\perp\Sigma^{1/2}\hat\theta_t}^2\vphantom{\sum^T}}.
  \end{align*}
  This is a quadratic inequality in the two terms on the left-hand side, and so by applying \propref{prop:solve-quad-ineqs},
  \begin{align*}
    \frac{1}{T}\sum_{t \in [T]}\norm[2]{P^\perp\Sigma^{1/2}B^\ast w_t^\ast}^2 &\lesssim  \frac{1}{T}\sum_{t \in [T]}\norm[2]{P^\perp\Sigma^{1/2}(\theta_t^\ast - \hat\theta_t)}^2 + \frac{1}{T}\sum_{t \in [T]}\norm[2]{P\Sigma^{1/2}(\theta_t^\ast - \hat\theta_t)}^2 \\
      &\qquad + \frac{1}{T}\sum_{t \in [T]}\norm[2]{\Sigma^{1/2}(\theta_t^\ast - \hat\theta_t)}^2 \\
      &\lesssim \frac{1}{T}\sum_{t \in [T]}\norm[2]{\Sigma^{1/2}(\theta_t^\ast - \hat\theta_t)}^2,
  \end{align*}
  where the last line follows by orthogonality.
  Finally, by \propref{prop:mat-to-proj},
  \[
    \frac{1}{T}\sum_{t \in [T]}\norm[2]{P^\perp\Sigma^{1/2}B^\ast w_t^\ast}^2 = \frac{1}{T}\norm[F]{P^\perp\Sigma^{1/2}B^\ast W^\ast}^2 \geq \frac{\sigma_k(W^\ast)^2}{T}\norm[F]{P_{\Sigma^{1/2}B_0}^\perp\Sigma^{1/2}B^\ast}^2,
  \]
  which together with the diversity assumption in \assumpref{assump:lin-diversity-cond} yields the final bound
  \[
    \norm[F]{P_{\Sigma^{1/2}B_0}^\perp\Sigma^{1/2}B^\ast}^2 \lesssim k\left[\frac{1}{T}\sum_{t \in [T]}\norm[2]{\Sigma^{1/2}(\theta_t^\ast - \hat\theta_t)}^2\right]. \qedhere
  \]
\end{proof}


==> results/nonlinear/hardcase/ermLearnsWrongNeurons.tex <==
\begin{restatable}[\frzrep{} learns incorrect neurons]{lemma}{ermLearnsWrongNeurons}
  \label{lemma:erm-learns-wrong-neurons}
  Fix an orthogonal matrix $A^\ast \in \reals^{d \times k}$ with $\col{A^\ast} \subseteq E^\ast$, and assume that we sample tasks from the distribution in \eqnref{eqn:relu-task-dist}.
  Assume that $\hat{B} = [\hat{A}, -\hat{A}]$ is the representation found by \frzrep{}.
  Then, with infinitely many tasks and per-task samples (\textit{i.e.} $n_\source, T \to \infty$), $\hat{A} = \col{E_k}$.
\end{restatable}
\begin{proof}
  Intuitively, the result follows from the fact that the optimal predictor is equivalent to a linear predictor, and thus the result follows by \lemmaref{lemma:erm-learns-wrong-space}.
  More formally, by \lemmaref{lemma:opt-relu-predictor-is-linear},
  \begin{align*}
    \meanloss(B) &= \frac{1}{T}\sum_{t \in [T]}\min_{w}\expt{(w^\top(Bx)_+ - x^\top\theta_t^\ast)^2} = \frac{1}{T}\sum_{t \in [T]}\min_{v}\expt{(x^\top Av - x^\top\theta_t^\ast)^2} \\
      &= \frac{1}{T}\sum_{t \in [T]}\min_v\norm[2]{\Sigma^{1/2}(Av - \theta_t^\ast)}^2 = \frac{1}{T}\sum_{t \in [T]}\norm[2]{P_{\Sigma^{1/2}A}^\perp\Sigma^{1/2}\theta_t^\ast}^2.
  \end{align*}
  At this point, we recognize that the objective is equivalent to the one analyzed in \lemmaref{lemma:erm-learns-wrong-space}, and thus the same characterization of global optima holds.
  That is, the solution $\hat{B}$ found by \frzrep{} can be expressed as $\hat{B} = [\hat A, -\hat A]$, where $\col{\hat A} = E_k$.
\end{proof}


==> results/nonlinear/hardcase/ermReLUMinimaxBound.tex <==
\begin{restatable}[\frzrep{} Minimax Bound, ReLU]{theorem}{ermReLUMinimaxBound}
  \IfAppendix{
    For an orthogonal matrix $A^\ast \in \reals^{d \times k}$ such that $\col{A^\ast} \subset E^\ast$, let $S_{A^\ast}$ be the set
    \[
      S_{A^\ast} = \set{\frac{1}{\sqrt{2\epsilon}}A^\ast v + \delta \suchthat \norm[2]{v} \leq 1, \norm[2]{\delta} \leq 1, \delta \in E_k}.
    \]
    We consider the following procedure:
    \begin{enumerate}
      \item We draw $n_\target$ samples for target time training, which are collected into a matrix $X$.
      \item Player chooses target-time estimator $x \mapsto \hat{w}^\top(\bar{B}^\top x) + \ind{x^\top\bar{B} \geq 0}\hat\Delta^\top x$, where $\bar{B}$, $\hat{w}$ and $\hat\Delta$ are measurable functions of $(X, y)$, and $\bar{B}$ is an orthogonal matrix with $\col{\bar{B}} = \col{\hat{B}}$.
      \item Adversary chooses an orthogonal matrix $A^\ast \in \reals^{d \times k}$ satisfying $\col{A^\ast} \subset E_k$, and a target time predictor $\theta^\ast \in S_{A^\ast}$.
      \item Compute the representation $\hat{B}$ returned by \frzrep{} under the setting of \lemmaref{lemma:erm-learns-wrong-neurons} with the task distribution determined by $A^\ast$.
      \item Target time samples are generated using $y \sim \gaussian{X\theta^\ast, \sigma^2I_n}$, and the player estimator is evaluated.
    \end{enumerate}
    Then, with probability at least $1 - \delta$ over the draw of $X$, we have that
    \[
      \min_{\bar{B}, \hat{w}, \hat{\Delta}}\max_{\substack{A^\ast \\ \theta^\ast \in S_{A^\ast}}}\expt{\frac{1}{n_\target}\sum_{i=1}^{n_\target}\left(x_i^\top\theta^\ast - \hat{w}^\top(\bar{B}^\top x_i) - \ind{x_i^\top\bar{B} > 0}\hat\Delta^\top x\right)^2} \gtrsim \frac{\sigma^2 d}{n_\target},
    \]
    where the expectation is over the randomness in the labels $y \sim \gaussian{X\theta^\ast, \sigma^2I_{n_\target}}$.
  }{
    For an orthogonal matrix $A^\ast \in \reals^{d \times k}$ such that $\col{A^\ast} \subset E^\ast$, let $B^\ast = [A^\ast, -A^\ast]$, and define $S_{A^\ast}$ to be the set
    \[
      S_{A^\ast} = \set{\frac{1}{\sqrt{2\epsilon}}A^\ast v + \delta \suchthat \norm[2]{v} \leq 1, \norm[2]{\delta} \leq 1, \delta \in E_k}.
    \]
    Furthermore, let $\hat{B}$ be the output of \frzrep{} with access to infinite per-task samples and tasks, with the task distribution deterined by $B^\ast$.
    Then, with high probability over the draw of $n_T \gg d$ samples during target training, we have that
    \begin{align*}
      &\min_{\bar{B}, \hat{w}, \hat\Delta}\max_{\substack{A^\ast \\ \theta^\ast \in S_{A^\ast}}}\expt{\frac{1}{n_\target}\norm[2]{X\theta^\ast - f_{(\bar{B} + \hat\Delta, \hat w)}(X)}^2} \gtrsim \frac{\sigma^2 d}{n_\target},
    \end{align*}
    where $\bar{B}$, $\hat{w}$, and $\hat\Delta$ are all measurable functions of $(X, y)$ to $\reals^{d \times 2k}$, $\reals^{2k}$, and $\reals^{d \times 2k}$, respectively, and $\col{\bar{B}} = \col{\hat{B}}$.
    Furthermore, the expectation is over the randomness in the labels $y \sim \gaussian{X\theta^\ast, \sigma^2I_{n_\target}}$.
  }
\end{restatable}
\begin{proof}
  Throughout this proof, we assume the high-probability event in \lemmaref{lemma:lin-targ-cov-concentration}, which guarantees that with probability at least $1 - \delta$,
  \[
    0.9\Sigma \preceq \frac{1}{n_\target}X^\top X \preceq 1.1\Sigma.
  \]

  Let $S$ denote the intersection of the $d$-dimensional unit sphere with $E_k$.
  For any infinite-dimensional vector $f$ indexed by $S$ and a measure $\mu$ on $S$, we define $\mu^\top f$ to denote integration with respect to $\mu$, i.e.
  \[
    \mu^\top f = \int_{S} f \ \diff{\mu}.
  \]
  We then define the infinite-dimensional vectors $\eta$ and $\zeta^{(i)}$ for $i = 1, \dots, d$, both indexed by $S$, as
  \[
    \eta(x) \defas (v^\top x)_+ \quad \text{and} \quad \zeta^{(i)}(x) \defas \ind{v^\top x > 0}x_i.
  \]
  Recall that by \lemmaref{lemma:erm-learns-wrong-neurons}, $\col{\hat{B}} = E_k$.
  With the preceding discussion in mind, we can equivalently think of the player as choosing $d + 1$ signed measures $\alpha$, $\beta_1, \dots, \beta_d$ over $S$, all with a common support of $2k$ elements in $S$, as a function of $(X, y)$.
  The player then plays the predictor
  \[
    x \mapsto \alpha^\top\eta(x) + \sum_{i=1}^{d}\beta_i^\top\zeta^{(i)}(x).
  \]
  Then, if we let $T = \set{\theta \suchthat \norm[2]{P_{E^\ast}\theta}^2 \leq 1/2\epsilon, \norm[2]{P_{E_k}\theta}^2 \leq 1} \subseteq S_{A^\ast}$, then we have the inequality
  \begin{align*}
    &\min_{\hat{w}, \hat{\Delta}}\max_{\substack{A^\ast \\ \theta^\ast \in S_{A^\ast}}}\expt{\frac{1}{n_\target}\sum_{i=1}^{n_\target}\left(x_i^\top\theta^\ast - \hat{w}^\top(\hat{B}^\top x_i)_+ - \ind{x_i^\top\hat{B} > 0}\hat\Delta^\top x\right)^2} \\
      &\qquad = \min_{\alpha, \beta_1, \dots, \beta_d}\max_{\substack{A^\ast \\ \theta^\ast \in S_{A^\ast}}}\expt{\frac{1}{n_\target}\sum_{i=1}^{n_\target}\left(x_i^\top\theta^\ast - \alpha^\top\eta(x) - \sum_{j=1}^{d}\beta_j^\top\zeta^{(j)}(x)\right)^2} \\
      &\qquad = \min_{\alpha, \beta_1, \dots, \beta_d}\max_{\theta^\ast \in T}\expt{\frac{1}{n_\target}\sum_{i=1}^{n_\target}\left(x_i^\top\theta^\ast - \alpha^\top\eta(x) - \sum_{j=1}^{d}\beta_j^\top\zeta^{(j)}(x)\right)^2},
  \end{align*}
  where the second equality follows from the fact that the expression has no direct dependence on $A^\ast$.

  The rest of the argument follows makes use of Fano's minimax bound, applied similarly as in the linear setting.
  First, note that for any $\theta \in T$, there exists $d + 1$ signed measures on $S$ with common support size $2k$, which we denote with $\alpha^{\theta}$ and $\beta_1^{\theta}, \dots, \beta_d^{\theta}$, such that $x^\top\theta = (\alpha^\theta)^\top\eta(x) + \sum_{j}(\beta_j^\theta)^\top\zeta^{(j)}(x)$.
  Using this construction, we can lift the local packing set from the linear setting into this setting, where the associated seminorm (defined over vector measures) is given by
  \[
    \norm{(\alpha, \beta_1, \dots, \beta_d)}^2 = \frac{1}{n_\target}\sum_{i=1}^{n_\target}\left(\alpha^\top\eta(x) + \sum_{j=1}^d\beta_j^\top\zeta^{(j)}(x)\right)^2.
  \]

  More formally, let $B$ be the unit ball under the $\Sigma$-norm, which we observe satisfies $(1/\sqrt{2})B \subseteq T$.
  Recall that there exists a $(1/2)$-packing of the unit $\Sigma$-ball in the $\Sigma$-norm with at least $2^d$ elements, via a standard volumetric argument - let this set be $P$.
  Equivalently, there exists a $(2\delta/\sqrt{0.9})$-packing of $(4\delta/\sqrt{0.9})B$ with at least $2^d$ elements, which we denote as $P$.
  Note that for any $\theta, \theta' \in P$,
  \[
    \norm{(\alpha^\theta, \beta_1^\theta, \dots, \beta_d^\theta) - (\alpha^{\theta'}, \beta_1^{\theta'}, \dots, \beta_d^{\theta'})}^2 = \frac{1}{n_\target}\norm[2]{X(\theta - \theta')}^2 \geq 0.9\norm[\Sigma]{\theta - \theta'}^2 > 4\delta^2,
  \]
  which implies that the vector measures corresponding to the elements of $P$ are $2\delta$-separated in the associated seminorm.
  Furthermore, for any $\theta, \theta' \in P$,
  \[
    \KL{\gaussian{X\theta, \sigma^2I_{n_\target}}}{\gaussian{X\theta', \sigma^2I_{n_\target}}} = \frac{1}{2\sigma^2}\norm[2]{X(\theta - \theta')}^2 \lesssim \frac{n_\target}{2\sigma^2}\norm[\Sigma]{\theta - \theta'}^2 \leq \frac{32n_\target}{0.9\sigma^2}\delta^2.
  \]
  Therefore, for any $\delta^2 \leq 1/32$, which ensures that $P \subseteq 4\delta B \subseteq (1/\sqrt{2})B \subseteq T$, Fano's inequality implies that
  \begin{align*}
    \min_{\alpha, \beta_1, \dots, \beta_d}\max_{\theta^\ast \in T}\expt{\norm{(\alpha^{\theta^\ast}, \beta_1^{\theta^\ast}, \dots, \beta_d^{\theta^\ast}) - (\alpha, \beta_1, \dots, \beta_d)}^2} &\geq \delta^2\left(1 - \frac{32n_\target}{0.9\sigma^2\log 2}\delta^2 - \frac{1}{d}\right) \\
      &\geq \delta^2\left(\frac{3}{4} - \frac{32n_\target}{0.9\sigma^2d\log 2}\delta^2\right).
  \end{align*}
  Therefore, as long as $n_\target \geq \left(\frac{0.9\log 2}{2}\right)\sigma^2 d$, we can set $\delta^2 = \left(\frac{0.9\log 2}{64}\right)\frac{\sigma^2d}{n_\target}$, which implies that
  \[
    \min_{\hat{w}, \hat{\Delta}}\max_{\substack{A^\ast \\ \theta^\ast \in S_{A^\ast}}}\expt{\frac{1}{n_\target}\sum_{i=1}^{n_\target}\left(x_i^\top\theta^\ast - \hat{w}^\top(\bar{B}^\top x_i) - \ind{x_i^\top\bar{B} > 0}\hat\Delta^\top x\right)^2} \gtrsim \frac{\sigma^2 d}{n_\target}. \qedhere
  \]
\end{proof}


==> results/nonlinear/hardcase/optReLUPredictorIsLinear.tex <==
\begin{restatable}[Optimal ReLU Predictor is Linear]{lemma}{optReLUPredictorIsLinear}
  \label{lemma:opt-relu-predictor-is-linear}
  Let $\theta \in \reals^d$, and assume that $B = [A, -A]$.
  Then, if we set
  \[
    w = \argmin_{w \in \reals^{2k}}\expt{(w^\top(B^\top x)_+ - x^\top\theta_t^\ast)^2},
  \]
  then the predictor $x \mapsto w^\top (B^\top x)$ is in fact a linear function of $x$, and takes the form of $x^\top Av$ for some $v \in \reals^k$.
\end{restatable}
\begin{proof}
  Write $w = [w_+, w_-]$, and thus the objective defining $w$ can be written as
  \[
    \min_{w_+, w_- \in \reals^k}\expt{(w_+^\top(A^\top x)_+ + w_-^\top(-A^\top x)_+ - x^\top\theta_t^\ast)^2}.
  \]
  Now, define the matrices
  \begin{align*}
    \Omega &\defas \expt{(A^\top x)_+(x^\top A)_+} = \expt{(-A^\top x)_+(-x^\top A)_+} \\
    \Gamma &\defas \expt{(-A^\top x)_+(x^\top A)_+} = \expt{(A^\top x)_+(-x^\top A)_+},
  \end{align*}
  where the equalities follow from the fact that $Ax$ and $-Ax$ are equal in distribution.
  Additionally,,
  \[
    \expt{(A^\top x)_+x^\top} = \frac{1}{2}\expt{(A^\top x)_+x^\top} - \frac{1}{2}\expt{(-A^\top x)_+x^\top} = \frac{1}{2}A^\top\expt{xx^\top} = \frac{1}{2}A^\top\Sigma,
  \]
  and thus once again since $Ax$ and $-Ax$ are equal in distribution,
  \[
    \expt{(-A^\top x)_+x^\top} = -\expt{(A^\top x)_+x^\top} = -\frac{1}{2}A^\top\Sigma.
  \]
  Thus, by explicitly solving for the optimum of the convex objective,
  \begin{align*}
    \begin{bmatrix}
      w_+ \\
      w_-
    \end{bmatrix}
    &=
    \frac{1}{2}
    \begin{bmatrix}
      \Omega & \Gamma \\
      \Gamma & \Omega \\
    \end{bmatrix}^{-1}
    \begin{bmatrix}
      A^\top\Sigma\theta_t^\ast \\
      -A^\top\Sigma\theta_t^\ast \\
    \end{bmatrix}
    \\
    &=
    \begin{bmatrix}
      (\Omega - \Gamma\Omega\Gamma)^{-1} & 0 \\
      0 & (\Omega - \Gamma\Omega\Gamma)^{-1} \\
    \end{bmatrix}
    \begin{bmatrix}
      I & -\Gamma\Omega^{-1} \\
      -\Gamma\Omega^{-1} & I \\
    \end{bmatrix}
    \begin{bmatrix}
      A^\top\Sigma\theta_t^\ast \\
      -A^\top\Sigma\theta_t^\ast \\
    \end{bmatrix},
  \end{align*}
  where we have applied blockwise matrix inversion to obtain the second inequality.
  From this, we see that $w_+ = w_-$, and thus the corresponding optimal predictor is linear, and can be shown to be $x \mapsto x^\top Aw_+$.
\end{proof}


==> results/nonlinear/hardcase/reLUAdaptTargPerf.tex <==
\begin{restatable}[Adaptation target performance, ReLU]{lemma}{reLUAdaptTargPerf}
  Let $B_0 = [A_0, -A_0]$, and fix a $\theta^\ast \in S_{A^\ast}$.
  Consider a learner which solves
  \[
    \min_{B}\min_{\substack{(w_t, \Delta_t) \\ \norm[F]{\Delta_t} \leq 1}}\frac{1}{n_\source}\sum_{t \in [T]}\norm[2]{\rho_{B}(X)[w, \Delta] - y}^2.
  \]
  during source training, and
  \[
    \min_{\substack{w, \Delta \\ \norm[F]{\Delta} \leq 1}}\frac{1}{n_\target}\norm[2]{\rho_{B_0}(X)[w, \Delta] - y}^2
  \]
  during target training, where $B_0$ is the representation obtained from source training.%
  \IfAppendix{
    Then, with probability at least $1 - \delta$,
    \begin{align*}
      \frac{1}{n_\target}\norm[2]{\rho_{B_0}(X)[w, \Delta] - X\theta^\ast}^2 &\lesssim \norm[2]{P_{\Sigma^{1/2}A_0}^\perp\Sigma^{1/2}A^\ast}^2 + \frac{\sigma^2 k}{n_\target}\left(1 + \log\frac{1}{\delta}\right) \\
      &\qquad + \frac{\sigma}{\sqrt{n_\target}}\sqrt{k\tr\Sigma\left(1 + \log\frac{1}{\delta}\right)}.
    \end{align*}
    In particular, with $k = \Theta(1)$ and $\epsilon = k/d$, and assuming access to infinite per-task samples and tasks during source training, the learner achieves target loss bounded as
    \begin{align*}
      \frac{1}{n_\target}\norm[2]{\rho_{B_0}(X)[w, \Delta] - X\theta^\ast}^2 \lesssim \frac{\sigma^2}{n_\target}\left(1 + \log\frac{1}{\delta}\right) + \frac{\sigma}{\sqrt{n_\target}}\sqrt{1 + \log\frac{1}{\delta}}
    \end{align*}
    with probability at least $1 - \delta$ over the draw of target samples.
  }{
    Finally, we set $k = \Theta(1)$ and $\epsilon = k/d$.
    Then, with access to infinite per-task samples and tasks during source training, the learner achieves target loss bounded as
    \begin{align*}
      &\frac{1}{n_\target}\norm[2]{\rho_{B_0}(X)[w, \Delta] - X\theta^\ast}^2 \\
        &\lesssim \frac{\sigma^2}{n_\target}\left(1 + \log\frac{1}{\delta}\right) + \frac{\sigma}{\sqrt{n_\target}}\sqrt{1 + \log\frac{1}{\delta}}
    \end{align*}
    with probability at least $1 - \delta$ over the draw of target samples.
  }
\end{restatable}
\begin{proof}
  Throughout the proof, we instantiate the high-probability event in \lemmaref{lemma:lin-targ-cov-concentration}, which guarantees that with probability at least $1 - \delta/9$,
  \[
    0.9\Sigma \preceq \frac{1}{n_\target}X^\top X \preceq 1.1\Sigma.
  \]

  By forming the least-squares basic inequality, we have that
  \begin{align*}
    &\frac{1}{n_\target}\norm[2]{\rho_{B_0}(X)[w, \Delta] - X(A^\ast v^\ast + \delta^\ast)}^2 \\
      &\qquad \lesssim \underbrace{\frac{1}{n_\target}\norm[2]{P_{XA_0}^\perp XA^\ast v^\ast}^2}_{\asdef \zeta} + \frac{1}{n_\target}\abs{\inprod{z, \rho_{B_0}(X)[w, \Delta] - P_{XA_0}XA^\ast v^\ast - X\delta^\ast}}.
  \end{align*}
  Then, since $P_{XA_0}XA^\ast v^\ast$ is in the span of $\phi_{B_0}(X)$, we can bound the right-hand side of the basic inequality by
  \begin{align*}
    &\zeta + \frac{1}{n_\target}\abs{\inprod{z, \smash{\underbrace{P_{\phi_{B_0}(X)}\left(\rho_{B_0}(X)[w, \Delta] - P_{XA_0}XA^\ast v^\ast - X\delta^\ast\right)}_{\asdef T_{\text{low-rank}}}}\vphantom{P^\perp_{\phi_{B_0}}}}}\vphantom{\underbrace{A}_{B_C}} \\ &\qquad + \frac{1}{n_\target}\abs{\inprod{z, P_{\phi_{B_0}(X)}^\perp\left(\psi_{B_0}(X)[\Delta] - X\delta^\ast\right)}}.
  \end{align*}
  Furthermore, we can lower bound the left-hand side by
  \[
    \frac{1}{n_\target}\norm[2]{\rho_{B_0}(X)[w, \Delta] - X(A^\ast v^\ast + \delta^\ast)}^2 \geq \frac{1}{n_\target}\norm[2]{T_{\text{low-rank}}}^2 + \frac{2}{n_\target}\inprod{P_{XA_0}^\perp XA^\ast v^\ast, T_{\text{low-rank}}}.
  \]
  Note that $\phi_{B_0}(X)$ is a matrix with rank $\leq 2k$, and therefore, $P_{\phi_{B_0}}(X)z$ is a chi-squared random variable, with at most $2k$ degrees of freedom.
  Subsequently, by applying known bounds on chi-squared random variables, we have that with probability at least $1 - (4/9)\delta$,
  \begin{align*}
    \frac{1}{n_\target}\norm[2]{T_{\text{low-rank}}}^2 &\leq \zeta + \left(\sqrt{\zeta} + \frac{2\sigma k}{\sqrt{n_\target}}\sqrt{1 + \log\frac{1}{\delta}}\right)\frac{1}{\sqrt{n_\target}}\norm[2]{T_{\text{low-rank}}} \\
      &\qquad + \frac{1}{n_\target}\abs{\inprod{z, P_{\phi_{B_0}(X)}^\perp\left(\psi_{B_0}(X)[\Delta] - X\delta^\ast\right)}},
  \end{align*}
  which thus implies via \propref{prop:solve-quad-ineqs} that
  \begin{align*}
    &\frac{1}{n_\target}\norm[2]{\rho_{B_0}(X)[w, \Delta] - X(A^\ast v^\ast + \delta^\ast)}^2 \\
      &\qquad \lesssim \zeta + \frac{\sigma^2k}{n_\target}\left(1 + \log\frac{1}{\delta}\right) + \frac{1}{n_\target}\abs{\inprod{z, P_{\phi_{B_0}(X)}^\perp\left(\psi_{B_0}(X)[\Delta] - X\delta^\ast\right)}}.
  \end{align*}
  To bound the final term, note that
  \begin{align*}
    &\frac{1}{n_\target}\abs{\inprod{z, P_{\phi_{B_0}(X)}^\perp\left(\psi_{B_0}(X)[\Delta] - X\delta^\ast\right)}} \\
    &\qquad \leq \frac{1}{\sqrt{n_\target}}\left[\norm[2]{\frac{1}{\sqrt{n_\target}}\psi_{B_0}(X)^\top P_{\phi_{B_0}(X)}^\perp z} + \norm[2]{\frac{1}{\sqrt{n_\target}}X^\top P_{\phi_{B_0}(X)}^\perp z}\right],
  \end{align*}
  by applying the norm bounds on $\Delta$ and $\delta^\ast$, and thus by applying the Hanson-Wright inequality, with probability at least $1 - (4/9)\delta$,
  \begin{align*}
    &\frac{1}{n_\target}\abs{\inprod{z, P_{\phi_{B_0}(X)}^\perp\left(\psi_{B_0}(X)[\Delta] - X\delta^\ast\right)}} \\
    &\qquad \leq \frac{\sigma}{\sqrt{n_\target}}\left[\sqrt{\frac{1}{n_\target}\tr \psi_{B_0}(X)^\top\psi_{B_0}(X)} + \sqrt{\frac{1}{n_\target}\tr X^\top X}\right]\sqrt{1 + \log\frac{1}{\delta}} \\
    &\qquad \lesssim \frac{\sigma}{\sqrt{n_\target}}\sqrt{k\tr\Sigma\left(1 + \log\frac{1}{\delta}\right)}.
  \end{align*}
  Therefore, since $\norm[2]{v^\ast} \leq 1$, we have an overall bound of
  \begin{align*}
    \frac{1}{n_\target}\norm[2]{\rho_{B_0}(X)[w, \Delta] - X\theta^\ast}^2  &\lesssim \norm[2]{P_{\Sigma^{1/2}A_0}^\perp\Sigma^{1/2}A^\ast}^2 + \frac{\sigma^2 k}{n_\target}\left(1 + \log\frac{1}{\delta}\right) \\
    &\qquad + \frac{\sigma}{\sqrt{n_\target}}\sqrt{k\tr\Sigma\left(1 + \log\frac{1}{\delta}\right)}.
  \end{align*}

  To prove the second part of the statement, note that with infinite source tasks and samples, global optimality with respect to the source loss together with \lemmaref{lemma:relu-transfer-lemma} implies that
  \[
    \frac{1}{T}\norm[F]{P_{\Sigma^{1/2} A_0}^\perp\Sigma^{1/2}A^\ast V^\ast}^2 = 0 \implies \norm[2]{P_{\Sigma^{1/2} A_0}^\perp\Sigma^{1/2}A^\ast} = 0,
  \]
  since $(k/T)\left[{V^\ast}^\top V^\ast\right] = I_k$.
  Furthermore, with the choice of $d$ and $\epsilon$, $\tr\Sigma = \Theta(1)$.
  Therefore, we obtain the second claim.
\end{proof}


==> results/nonlinear/hardcase/reLUTransferLemma.tex <==
\begin{restatable}[Transfer Lemma, ReLU]{lemma}{reLUTransferLemma}
  \label{lemma:relu-transfer-lemma}
  Assume that $B_0 = [A_0, -A_0]$.
  Then, we have that
  \[
    \frac{1}{T}\norm[F]{P_{\Sigma^{1/2}A_0}^\perp \Sigma^{1/2}A^\ast W^\ast}^2 \lesssim \frac{1}{T}\sum_{i=1}^{T}\min_{w, \Delta}\expt{\left(x^\top\theta_t^\ast - \rho_{B_0}(x)[w, \Delta]\right)^2}.
  \]
\end{restatable}
\begin{proof}
  This proof follows the outline of \lemmaref{lemma:lin-transfer-lemma}, with all inner products computed with respect to $\inprod{\cdot, \cdot}_{L_2}$.
  Throughout the proof, we will write $P$ and $P^\perp$ as shorthand for the operators $P_{\phi_{B_0}}$ and $P_{\phi_{B_0}}^\perp$, respectively.
  First, we decompose the task-averaged population risk as for any choices of $(w_t), (\Delta_t)$ as
  \begin{align*}
    &\frac{1}{T}\sum_{i=1}^{T}\norm[L_2]{(\cdot)^\top\theta_t^\ast - \rho_{B_0}(\cdot)[w_t, \Delta_t]}^2 \\
      &\qquad \gtrsim \frac{1}{T}\sum_{t \in [T]}\norm[L_2]{\phi_{B^\ast}(\cdot)^\top w_t^\ast - [P\rho_{B_0}](\cdot)[w_t, \Delta_t]}^2 \\
      &\qquad\qquad + \frac{1}{T}\sum_{t \in [T]}\norm[L_2]{\psi_{B^\ast}(\cdot)^\top \Delta_t^\ast - [P^\perp\rho_{B_0}](\cdot)[w_t, \Delta_t]}^2 \\
      &\qquad\qquad - \frac{1}{T}\sum_{t \in [T]}\abs{\inprod{\phi_{B^\ast}(\cdot)^\top w_t^\ast - [P\rho_{B_0}](\cdot)[w_t, \Delta_t], \psi_{B^\ast}(\cdot)^\top \Delta_t^\ast - [P^\perp\rho_{B_0}](\cdot)[w_t, \Delta_t]}_{L_2}} \\
      &\qquad \gtrsim \frac{1}{T}\sum_{t \in [T]}\norm[2]{P_{\Sigma^{1/2}A_0}^\perp\Sigma^{1/2}A^\ast v_t^\ast}^2 + \frac{1}{T}\sum_{t \in [T]}\norm[L_2]{\psi_{B^\ast}(\cdot)^\top \Delta_t^\ast - [P^\perp\rho_{B_0}](\cdot)[w_t, \Delta_t]}^2 \\
      &\qquad\qquad - \frac{1}{T}\sum_{t \in [T]}\abs{\inprod{\phi_{B^\ast}(\cdot)^\top w_t^\ast - [P\rho_{B_0}](\cdot)[w_t, \Delta_t], \psi_{B^\ast}(\cdot)^\top \Delta_t^\ast - [P^\perp\rho_{B_0}](\cdot)[w_t, \Delta_t]}_{L_2}}.
  \end{align*}
  The second inequality follows from noting that $\phi_{B^\ast}(x)^\top w_t^\ast$ is a linear function of $x$, and thus by \lemmaref{lemma:opt-relu-predictor-is-linear}, the best linear predictor on $\phi$ is a linear function of $x$.
  Since the $L_2$-norm on linear functions of $x$ is equivalent to the $\Sigma$-norm on the parameters, we obtain the inequality above\footnote{This is exactly the argument used in \lemmaref{lemma:lin-transfer-lemma}.}.

  Now, we proceed to prove a bound on the inner product above.
  For any fixed $t \in [T]$,
  \begin{align*}
    &\abs{\inprod{\phi_{B^\ast}(\cdot)^\top w_t^\ast - [P\rho_{B_0}](\cdot)[w, \Delta], \psi_{B^\ast}(\cdot)^\top \Delta_t^\ast - [P^\perp\rho_{B_0}](\cdot)[w, \Delta]}_{L_2}} \\
    &\qquad \leq \abs{\inprod{\phi_{B^\ast}(\cdot)^\top w_t^\ast - [P\rho_{B^\ast}](\cdot)[w_t^\ast, \Delta_t^\ast], \psi_{B^\ast}(\cdot)^\top \Delta_t^\ast - [P^\perp\rho_{B^\ast}](\cdot)[w_t^\ast, \Delta_t^\ast]}_{L_2}} \\
    &\qquad\qquad + \abs{\inprod{\phi_{B^\ast}(\cdot)^\top w_t^\ast - [P\rho_{B^\ast}](\cdot)[w_t^\ast, \Delta_t^\ast], [P^\perp\rho_{B^\ast}](\cdot)[w_t^\ast, \Delta_t^\ast] - [P^\perp\rho_{B_0}](\cdot)[w_t, \Delta_t]}_{L_2}} \\
    &\qquad\qquad + \abs{\inprod{[P\rho_{B^\ast}](\cdot)[w_t^\ast, \Delta_t^\ast] - [P\rho_{B_0}](\cdot)[w_t, \Delta_t], \psi_{B^\ast}(\cdot)^\top \Delta_t^\ast - [P^\perp\rho_{B_0}](\cdot)[w_t, \Delta_t]}_{L_2}} \\
    &\qquad \leq \abs{\inprod{\phi_{B^\ast}(\cdot)^\top w_t^\ast - [P\rho_{B^\ast}](\cdot)[w_t^\ast, \Delta_t^\ast], \psi_{B^\ast}(\cdot)^\top \Delta_t^\ast - [P^\perp\rho_{B^\ast}](\cdot)[w_t^\ast, \Delta_t^\ast]}_{L_2}} \\
    &\qquad\qquad + \abs{\inprod{[P^\perp\phi_{B^\ast}](\cdot)^\top w_t^\ast, [P^\perp\rho_{B^\ast}](\cdot)[w_t^\ast, \Delta_t^\ast] - [P^\perp\rho_{B_0}](\cdot)[w_t, \Delta_t]}_{L_2}} \\
    &\qquad\qquad + \abs{\inprod{[P\rho_{B^\ast}](\cdot)[w_t^\ast, \Delta_t^\ast] - [P\rho_{B_0}](\cdot)[w_t, \Delta_t], \psi_{B^\ast}(\cdot)^\top \Delta_t^\ast - [P^\perp\rho_{B_0}](\cdot)[w_t, \Delta_t]}_{L_2}},
  \end{align*}
  where adding and subtracting $[P\rho_{B^\ast}](\cdot)[w_t^\ast, \Delta_t^\ast]$ and $[P^\perp\rho_{B^\ast}](\cdot)[w_t^\ast, \Delta_t^\ast]$ in the first and second arguments of the inner product, respectively, results in the first inequality.
  The second inequality then uses the orthogonality properties of $P$ and $P^\perp$ in the second term.
  Furthermore, observe that
  \begin{align*}
    &\abs{\inprod{\phi_{B^\ast}(x)^\top w_t^\ast - [P\rho_{B^\ast}](x)[w_t^\ast, \Delta_t^\ast], \psi_{B^\ast}(x)^\top \Delta_t^\ast - [P^\perp\rho_{B^\ast}](x)[w_t^\ast, \Delta_t^\ast]}_{L_2}} \\
    &\qquad = \abs{\inprod{[P^\perp\phi_{B^\ast}](x)^\top w_t^\ast - [P\psi_{B^\ast}](x)^\top\Delta_t^\ast, [P^\perp\psi_{B^\ast}](x)^\top \Delta_t^\ast - [P\phi_{B^\ast}](x)[w_t^\ast, \Delta_t^\ast]}_{L_2}} \\
    &\qquad = \abs{\inprod{\phi_{B^\ast}(x)^\top w_t^\ast, \psi_{B^\ast}(x)^\top \Delta_t^\ast}_{L_2}} = \abs{w_t^\ast A^\ast\Sigma\delta_t^\ast} \\
    &\qquad = 0,
  \end{align*}
  where we have used the algebraically-verifiable fact that $[P\rho_{B^\ast}](\cdot)[w, \Delta] = [P\phi_{B^\ast}](x)^\top + [P\psi_{B^\ast}](x)[\Delta]$, and that $[P^\perp\rho_{B^\ast}][w, \Delta]$ decomposes in a similar fashion.
  Finally, since $\phi_B^\ast(x)^\top w_t^\ast$ is linear, we can apply \lemmaref{lemma:opt-relu-predictor-is-linear}, and thus
  \[
    \norm[L_2]{[P^\perp \phi_{B^\ast}](x)^\top w_t^\ast} = \norm[2]{P_{\Sigma^{1/2}A_0}^\perp\Sigma^{1/2}A^\ast v_t^\ast}.
  \]

  From here, we note that we have an analogous quadratic inequality to that of \lemmaref{lemma:lin-transfer-lemma} in the terms
  \[
    \frac{1}{T}\sum_{t \in [T]}\norm[2]{P_{\Sigma^{1/2}A_0}^\perp\Sigma^{1/2}A^\ast v_t^\ast}^2 \quad \text{and} \quad \frac{1}{T}\sum_{t \in [T]}\norm[L_2]{\psi_{B^\ast}(\cdot)^\top \Delta_t^\ast - [P^\perp\rho_{B_0}](\cdot)[w_t, \Delta_t]}^2
  \]
  upon applying Cauchy-Schwarz as before.
  Furthermore, note that via orthogonality, we have the Pythagorean identity
  \[
    \norm[L_2]{P\rho}^2 + \norm[L_2]{P^\perp\rho}^2 \leq \norm[L_2]{\rho}^2,
  \]
  and thus by following the exact same algebraic argument as in \lemmaref{lemma:lin-transfer-lemma} of using \propref{prop:solve-quad-ineqs},
  \begin{align*}
    \frac{1}{T}\norm[F]{P_{\Sigma^{1/2}A_0}^\perp\Sigma^{1/2}A^\ast V^\ast}^2 &= \frac{1}{T}\sum_{t \in [T]}\norm[2]{P_{\Sigma^{1/2}A_0}^\perp\Sigma^{1/2}A^\ast v_t^\ast}^2 \\ 
      &\leq \frac{1}{T}\sum_{t \in [T]}\expt{(x^\top\theta_t^\ast - \rho_{B_0}(x)[w_t, \Delta_t])^2}.
  \end{align*}
  Since the result holds for any $(w_t)$ and $(\Delta_t)$, it holds for the minimizers.
\end{proof}


==> results/nonlinear/logistic/logisticDiversityCondition.tex <==
\begin{restatable}[Diversity condition, logistic regression]{lemma}{logisticDiversityCondition}
  Under the assumptions above, the source tasks satisfy a $(\Omega(\exp[-\rho^3(r + \delta_0)\norm[2]{\Sigma}^{1/2}]), 0)$-diversity condition.
\end{restatable}
\begin{proof}
  We remark that under the choice of $q$ and the logistic loss, we have that
  \[
    \expt[x, y]{\ell(g_\theta(x), y) - \ell(g_{\theta'}(x), y)} = \expt[x]{\KL{\bernoulli{\sigma(g_\theta(x))}}{\bernoulli{\sigma(g_{\theta'}(x))}}}
  \]
  Using the results in \citet[Lemmas 2 and 3]{tripuraneni2020theory},
  \begin{align}
    \frac{1}{8}\expt[x]{\exp(-\max(\abs{g_{\theta}(x)}, \abs{g_{\theta'}(x)}))(g_{\theta}(x) - g_{\theta'}(x))^2} &\leq \expt[x, y]{\ell(g_\theta(x), y) - \ell(g_{\theta'}(x), y)} \label{eqn-int:logistic-lower-bound} \\
    \expt[x, y]{\ell(g_\theta(x), y) - \ell(g_{\theta'}(x), y)} &\leq \frac{1}{8}\expt[x]{(g_{\theta}(x) - g_{\theta'}(x))^2} \label{eqn-int:logistic-upper-bound}.
  \end{align}
  In what follows, we will make use of \eqnref{eqn-int:logistic-lower-bound} to lower bound the task-averaged best-case performance, and \eqnref{eqn-int:logistic-upper-bound} to upper bound the expected best-case target performance.
  Note that this results in bounds in terms of best-case mean squared error -- we can then proceed to use arguments similar to that of the linear case to connect the two inequalities.

  \vspace{2ex}
  \noindent
  \underline{Upper bounding the expected best-case target performance.}
  \vspace{1ex}

  Assume that the optimal predictor is given by $\theta^\ast = B^\ast w^\ast + \delta^\ast$.
  Then, defining
  \[
    \hat\Delta = \frac{1}{\beta}\delta^\ast w_0^\top \quad \text{and} \quad \bar{w} = \frac{1}{\beta}(B_0^\top\Sigma B_0)^\dagger B_0^\top\Sigma B^\ast w^\ast,
  \]
  we note that $\hat\delta \defas ([\hat\Delta, 0], [0, \bar{w}^\top]^\top) \in \constraintset_\target^\beta$, following the argument in \lemmaref{lemma:lin-opt-consts}, and achieves a squared-error excess risk of
  \[
    \expt{(\beta g_{\theta + \hat\delta}(x) - g_{\theta^\ast}(x))^2} = \norm[2]{\Sigma^{1/2}[(B_0\bar{w} + \delta^\ast) - (B^\ast w^\ast - \delta^\ast)]}^2 = \norm[2]{P_{\Sigma^{1/2}B_0}^\perp \Sigma^{1/2}B^\ast w^\ast}^2.
  \]
  Therefore, by taking the infimum of the excess risk over feasible $\delta$ and applying the excess risk upper bound in \eqnref{eqn-int:logistic-upper-bound},
  \begin{align*}
    \inf_{\delta \in \constraintset_\target^\beta}\expt[x, y]{\ell(\beta g_{\theta_0 + \delta}(x), y) - \ell(g_{\theta^\ast}(x), y)} &\leq \expt[x, y]{\ell(\beta g_{\theta_0 + \hat\delta}(x), y) - \ell(g_{\theta^\ast}(x), y)} \\
      &\leq \frac{1}{8}\expt{(\beta g_{\theta_0 + \hat\delta}(x) - g_{\theta^\ast}(x))^2} \\
      &\leq \frac{1}{8}\norm[2]{P_{\Sigma^{1/2}B_0}^\perp\Sigma^{1/2}B^\ast w^\ast}^2.
  \end{align*}
  Finally, recall that $\expt[\theta^\ast \sim \rho]{(w^\ast)(w^\ast)^\top} = (r^2/k)I$.
  Therefore, by taking expectations with respect to $\rho$,
  \begin{align*}
    &\expt[\theta^\ast \distas \rho]{\inf_{\delta \in \constraintset_\target^\beta}\expt[x, y]{\ell(\beta g_{\theta_0 + \delta}(x), y) - \ell(g_{\theta^\ast}(x), y)}} \\
      &\qquad \lesssim \expt[\theta^\ast \distas \rho]{\tr P_{\Sigma^{1/2}B_0}^\perp\Sigma^{1/2}B^\ast(w^\ast)(w^\ast)^\top\left(P_{\Sigma^{1/2}B_0}^\perp\Sigma^{1/2}B^\ast\right)^\top} \\
      &\qquad = \frac{r^2}{k}\norm[F]{P_{\Sigma^{1/2}B_0}^\perp\Sigma^{1/2}B^\ast}^2.
  \end{align*}

  \vspace{2ex}
  \noindent
  \underline{Lower bounding the task-averaged best-case performance.}
  \vspace{1ex}

  We proceed to lower bound the task-averaged best-case performance.
  To proof proceeds similarly to that of \citet{tripuraneni2020theory}, lower bounding the excess risk by a constant multiple of the squared-error excess risk.
  Then, the result follows by an application of the transfer lemma in \lemmaref{lemma:lin-transfer-lemma}.

  Fix a task $t \in [T]$.
  Define $Z_1 \defas x^\top(B^\ast w_t^\ast + \delta_t^\ast)$ and $Z_2 \defas x^\top(B_0w_t + \delta_t)$.
  We see that $Z_1$ is sub-Gaussian with parameter $\rho^2\norm[2]{\Sigma^{1/2}(B^\ast w_t^\ast + \delta_t^\ast)}^2 \leq \rho^2(r^2 + \delta_0^2)\norm[2]{\Sigma} \asdef \sigma^2$.
  Note that $Z_2$ is also sub-Gaussian with proxy $\sigma^2$.
  Then, by applying the lower bound in \eqnref{eqn-int:logistic-lower-bound-w-sg},
  \begin{equation}
    \label{eqn-int:logistic-lower-bound-w-sg}
    \expt[x, y]{\ell(g_{\hat\theta_t}(x), y) - \ell(g_{\theta_t^\ast}(x), y)} \geq \frac{1}{8}\expt[x]{e^{-\max(\abs{Z_1}, \abs{Z_2})}(g_{\hat\theta_t}(x) - g_{\theta_t^\ast}(x))^2}.
  \end{equation}
  We will now show that the right-hand side is lower bounded by a constant multiple of the squared error excess risk.
  Intuitively, since $Z_1$ and $Z_2$ concentrate around $0$, $e^{-\max(\abs{Z_1}, \abs{Z_2})}$ concentrates around $1$.

  Formally, consider the event $E_\alpha \defas \set{\max(\abs{Z_1}, \abs{Z_2}) \leq \alpha\sigma}$ for any $\alpha$.
  Since the quantity inside the expectation of \eqnref{eqn-int:logistic-lower-bound-w-sg} is non-negative,
  \begin{align*}
    &\frac{1}{8}\expt[x]{e^{-\max(\abs{Z_1}, \abs{Z_2})}(g_{\hat\theta_t}(x) - g_{\theta_t^\ast}(x))^2} \\
      &\qquad \geq \frac{1}{8}\expt{\ind{E_\alpha}e^{-\alpha\sigma}(g_{\hat\theta_t}(x) - g_{\theta_t^\ast}(x))^2} \\
      &\qquad \geq \frac{e^{-\alpha\sigma}}{8}\left\{\expt{(g_{\hat\theta_t}(x) - g_{\theta_t^\ast}(x))^2} - \expt{\ind{E_\alpha\complement}(g_{\hat\theta_t}(x) - g_{\theta_t^\ast}(x))^2}\right\}.
  \end{align*}
  Now, we upper bound the last term.
  By Cauchy-Schwarz,
  \[
    \expt{\ind{E_\alpha\complement}(g_{\hat\theta_t}(x) - g_{\theta_t^\ast}(x))^2} \leq \sqrt{\prob{E_\alpha\complement}}\sqrt{\expt{(g_{\hat\theta_t}(x) - g_{\theta_t^\ast}(x))^4}},
  \]
  where we have used the fact that $\var{X} \leq \sigma^2$ for a $\sigma^2$-sub-Gaussian random variable.
  We use properties of sub-Gaussian random variables to bound both factors.
  First, by Chebyshev's inequality,
  \[
    \prob{E_\alpha\complement} \leq 2\prob{\abs{Z_1} \geq \alpha\sigma} \leq \frac{2\var{Z_1}}{\alpha^2\sigma^2} \leq \frac{2}{\alpha^2}.
  \]
  For the second factor, $g_{\hat\theta_t}(x) - g_{\theta_t^\ast}(x)$ is sub-Gaussian with proxy $\rho^2\expt{(g_{\hat\theta_t}(x) - g_{\theta_t^\ast}(x))^2}$, and so via an equivalent definition of sub-Gaussian random variables,
  \[
    \sqrt{\expt{(g_{\hat\theta_t}(x) - g_{\theta_t^\ast}(x))^4}} \lesssim \rho^2\expt{(g_{\hat\theta_t}(x) - g_{\theta_t^\ast}(x))^2}.
  \]
  Putting these bounds together, we have that
  \[
    \expt{\ind{E_\alpha\complement}(g_{\hat\theta_t}(x) - g_{\theta_t^\ast}(x))^2} \lesssim \frac{\rho^2}{\alpha}\expt{(g_{\hat\theta_t}(x) - g_{\theta_t^\ast}(x))^2}.
  \]

  Therefore, by setting $\alpha \asymp \rho^2$, we can ensure that
  \begin{align*}
    &\expt[x, y]{\ell(g_{\hat\theta_t}(x), y) - \ell(g_{\theta_t^\ast}(x), y)} \gtrsim e^{-\rho^3(r + \delta_0)\norm[2]{\Sigma}^{1/2}}\expt{(x^\top\hat\theta_t - x^\top\theta_t^\ast)^2} \\
    &\implies \frac{1}{T}\sum_{t \in [T]}\expt[x, y]{\ell(g_{\hat\theta_t}(x), y) - \ell(g_{\theta_t^\ast}(x), y)} \\
    &\qquad\qquad \gtrsim \frac{e^{-\rho^3(r + \delta_0)\norm[2]{\Sigma}^{1/2}}}{T}\sum_{t \in [T]}\norm[2]{\Sigma^{1/2}(B_0w_t + \delta_{t} - B^\ast w_t^\ast + \delta_t^\ast)}^2.
  \end{align*}
  By applying \lemmaref{lemma:lin-transfer-lemma}, we finally obtain the final lower bound
  \begin{align*}
    &\frac{e^{\rho^3(r + \delta_0)\norm[2]{\Sigma}^{1/2}}}{T}\sum_{t \in [T]}\inf_{\delta_t \in \constraintset_\source}\expt[x, y]{\ell(g_{\theta_0 + \delta_t}(x), y) - \ell(g_{\theta_t^\ast}(x), y)} \geq \frac{r^2}{k}\norm[F]{P_{\Sigma^{1/2}B_0}^\perp\Sigma^{1/2}B^\ast}^2.
  \end{align*}

  Putting everything together, we thus have the desired diversity condition
  \begin{align*}
    &\inf_{\norm{\delta} \leq \delta_0}\expt[x, y]{\ell(\beta g_{\theta_0 + \delta}(x), y) - \ell(g_{\theta^\ast}(x), y)} \\
      &\qquad \lesssim \frac{e^{\rho^3(r + \delta_0)\norm[2]{\Sigma}^{1/2}}}{T}\sum_{t \in [T]}\inf_{\norm{\hat\delta_t} \leq \delta_0}\expt[x, y]{\ell(g_{\theta_0 + \hat\delta_t}(x), y) - \ell(g_{\theta_t^\ast}(x), y)}. \qedhere
  \end{align*}
\end{proof}


==> results/nonlinear/logistic/logisticPerformanceBound.tex <==
\begin{restatable}[Performance Guarantee for Logistic Regression]{theorem}{logisticPerformanceBound}
  \IfAppendix{
    Assume that \assumpref{assump:logistic-sg-inputs} and \assumpref{assump:logistic-diversity-cond} both hold.
    Set the parameters for target time training to be
    \[
      \beta = (\kappa r^2 + \delta_0^2)\max\left(1, \frac{\sqrt{\tr\Sigma}}{1/\delta\sqrt{n_\target}}\right) \quad \text{and} \quad T_\pgd = \frac{(\kappa r^2 + \delta_0^2)\tr\Sigma}{1/\delta^2n_\target}.
    \]
    Then, for $n_\source, n_\target \gtrsim \rho^4 d$, we have that with probability at least $1 - \delta$ over the random draw of samples, the iterates $(\theta_t)$ satisfy
    \begin{align*}
      &\expt[g^\ast \sim \rho]{\min_t\meanloss^{g^\ast}_\infty(g_{\theta_t}) - \meanloss_\infty^{g^\ast}(g^\ast)} \\
        &\quad \lesssim \frac{1}{\delta}\left\{r\kappa^{1/2}\norm[2]{\Sigma}^{1/2}\sqrt{\frac{k}{n_\target}} + \frac{\delta_0}{\sqrt{n_\target}}\sqrt{\tr\Sigma}\right. \\
        &\quad\qquad\qquad \left.+ \exp\left[\rho^3(r + \delta_0)\norm[2]{\Sigma}^{1/2}\right]\left[\frac{r\norm[2]{\Sigma}^{1/2}}{\sqrt{n_\source T}}\sqrt{kT + kd\log n_\source} + \frac{\delta_0}{\sqrt{n_\source}}\sqrt{\tr\Sigma}\right]\right\}.
    \end{align*}
  }{
    Assume that \assumpref{assump:logistic-sg-inputs} and \assumpref{assump:logistic-diversity-cond} both hold, and that $n_\source \geq n_\target \gtrsim \rho^4 d$.
    Then, there exists a setting of the training parameters (see \secref{sec:case-study-proofs}) so that with probability at least $1 - \delta$ over the random draw of samples, the iterates $(\theta_t)$ generated by PGD satisfy
    \begin{align*}
      &\expt[g^\ast \sim \rho]{\min_t\meanloss^{g^\ast}_\infty(g_{\theta_t}) - \meanloss_\infty^{g^\ast}(g^\ast)} \lesssim \frac{1}{\delta}\left[r\sqrt{\frac{k}{n_\target}} + \frac{\delta_0}{\sqrt{n_\target}}\sqrt{\tr\Sigma} + r\sqrt{\frac{kd}{n_\source T}}\right].
    \end{align*}
  }
\end{restatable}
\begin{proof}
  With probability at least $1 - \delta/2$, the approximate linearity property of the function class holds via \lemmaref{lemma:lin-targ-cov-concentration} and \lemmaref{lemma:lin-approx-linearity}.
  Therefore, by combining all prior calculations and instantiating \thmref{thm:general-performance-bound} with failure probability $\delta/2$, projected gradient descent finds a predictor $g$ satisfying the desired bound in the theorem statement.
\end{proof}


==> results/nonlinear/logistic/logisticSourceRademacher.tex <==
\begin{restatable}[Source Rademacher Bound]{lemma}{logisticSourceRademacher}
  Assume that $n_\source \gtrsim \rho^4d$.
  Then, we can bound the source Rademacher complexity as
  \[
    \frac{1}{T}\mathcal{R}_{n_\source}\left[\Union_{\theta \in \Theta_0}\adaptset_{\theta}^{\constraintset_\source}\right] \lesssim \frac{r\norm[2]{\Sigma}^{1/2}}{\sqrt{n_\source T}}\sqrt{kT + kd\log n_\source} + \frac{\delta_0}{\sqrt{n_\source}}\sqrt{\tr\Sigma}.
  \]
\end{restatable}
\begin{proof}
  Observe that if $(\Delta_t, w_t) \in \constraintset_\source$, then $\delta_t \defas \Delta_tw_t$ satifies $\norm[2]{\delta_t} \leq \delta_0$.
  Therefore, we have that
  \begin{align*}
    \frac{1}{T}\mathcal{R}_{n_\source}\left[\Union_{\theta \in \Theta_0}\adaptset_{\theta}^{\constraintset_\source}\right] &= \expt{\sup_{\substack{B \\ (\Delta_t, w_t) \in \constraintset_\source}}\frac{1}{n_\source T}\sum_{t \in [T]}\inprod{\epsilon_t, X_t(B + \Delta_t)w_t}} \\
      &= \underbrace{\expt{\sup_{\substack{B \\ \norm[2]{w_t} \leq r}}\frac{1}{n_\source T}\sum_{t \in [T]}\inprod{\epsilon_t, X_tBw_t}}}_{\asdef (\mathrm{I})} + \underbrace{\expt{\sup_{\norm[2]{\delta_t} \leq \delta_0}\frac{1}{n_\source T}\sum_{t \in [T]}\inprod{\epsilon_t, X\delta_t}}}_{\asdef (\mathrm{II})}
  \end{align*}
  We proceed to bound these two quantities separately.

  \vspace{2ex}
  \noindent
  \underline{Bounding (I) via discretization.}
  \vspace{1ex}

  In this section, we bound the complexity by discretizing the set $\mathcal{O}^{k \times d}$ of $(k \times d)$ orthogonal matrices.
  We remark that the argument is similar in form to that of \lemmaref{lemma:lin-source-train-bound}.

  Let $\mathcal{S}$ be an $\epsilon$-covering of $\mathcal{O}^{k \times d}$ in the Frobenius norm with at most $(6\sqrt{k}/\epsilon)^{dk}$ elements guaranteed by \propref{prop:orth-mat-covering}.
  Then,
  \begin{align*}
    (\mathrm{I}) \leq \underbrace{\expt{\sup_{\substack{B \in \mathcal{S} \\ \norm[2]{w_t} \leq r}}\frac{1}{n_\source T}\sum_{t \in [T]}\inprod{\epsilon_t, X_tBw_t}}}_{\asdef (\mathrm{A})} + \underbrace{\expt{\sup_{\substack{B, \bar{B} \in \mathcal{S} \\ \norm[F]{B - \bar{B}} \leq \epsilon \\ \norm[2]{w_t} \leq r}}\frac{1}{n_\source T}\sum_{t \in [T]}\inprod{\epsilon_t, X_t(B - \bar{B})w_t}}}_{\asdef (\mathrm{B})}
  \end{align*}
  To bound $(\mathrm{A})$, we bound the corresponding Gaussian complexity and use the fact that $\mathcal{R}(\cdot) \lesssim \mathcal{G}(\cdot)$.
  Consequently, via multiple applications of Cauchy-Schwarz,
  \begin{align*}
    (\mathrm{A}) &\leq \sqrt{\frac{\pi}{2}}\expt{\sup_{\substack{B \in \mathcal{S} \\ \norm[2]{w_t} \leq r}}\frac{1}{n_\source T}\sum_{t \in [T]}\inprod{P_{X_tB}z_t, X_tBw_t}} \\
      &\lesssim \sqrt{\expt{\sup_{B \in \mathcal{S}}\frac{1}{n_\source T}\sum_{t \in [T]}\norm[2]{P_{X_tB}z_t}^2}}\sqrt{\expt{\sup_{\substack{B \in \mathcal{S} \\ \norm[2]{w_t} \leq r}}\frac{1}{n_\source T}\sum_{t \in [T]}\norm[2]{X_tBw_t}^2}}.
  \end{align*}
  Conditioned on $X_t$, $\sum_{t \in [T]}\norm[2]{P_{X_tB}z_t}^2$ is distributed as a chi-squared random variable with $kT$ degrees of freedom, with mean $kT$.
  Therefore, using known bounds on expectations of finite maxima of subexponential random variables,
  \begin{equation}
    \label{eqn-int:logistic-finite-maxima-bound}
    \begin{aligned}
    &\expt{\sup_{B \in S}\sum_{t \in [T]}\norm[2]{P_{X_tB}z_t}^2 - kT} \lesssim \sqrt{kT\log\card{\mathcal{S}}} + \log\card{S} \\
    &\implies \expt{\sup_{B \in S}\sum_{t \in [T]}\norm[2]{P_{X_tB}z_t}^2} \lesssim kT + \log\card{S}.
    \end{aligned}
  \end{equation}
  Furthermore, by applying the expectation bound on the empirical spectral norm in \propref{prop:empirical-spec-norm-exp-bound},
  \begin{align}
    \sqrt{\expt{\sup_{\substack{B \in \mathcal{S} \\ \norm[2]{w_t} \leq r}}\frac{1}{n_\source T}\sum_{t \in [T]}\norm[2]{X_tBw_t}^2}} &= r\sqrt{\expt{\sup_{B \in \mathcal{S}}\frac{1}{T}\sum_{t \in [T]}\lambda_{\max}\left(\frac{B^\top X_t^\top X_tB}{n_\source}\right)}} \\
      &\leq r\sqrt{\expt{\lambda_{\max}\left(\frac{X_t^\top X_t}{n_\source}\right)}} \nonumber \\
      &\lesssim r\norm[2]{\Sigma}^{1/2}. \label{eqn-int:predictor-norm-bound}
  \end{align}
  Therefore, by combining the inequalities from \eqnref{eqn-int:logistic-finite-maxima-bound} and \eqnref{eqn-int:predictor-norm-bound},
  \[
    (\mathrm{A}) \lesssim \frac{\norm[2]{\Sigma}^{1/2}}{\sqrt{n_\source T}}\sqrt{kT + \log\card{S}}.
  \]

  We proceed to bound (B), the error arising from discretization.
  We have that
  \begin{align*}
    (\mathrm{B}) &\leq \expt{\sup_{\substack{B, \bar{B} \in \mathcal{S} \\ \norm[F]{B - \bar{B}} \leq \epsilon \\ \norm[2]{w_t} \leq r}}\frac{1}{n_\source T}\sum_{t \in [T]}\inprod{\epsilon_t, X_t(B - \bar{B})w_t}} \lesssim r\epsilon\norm[2]{\Sigma^{1/2}}.
  \end{align*}
  Finally, by setting $\epsilon = \sqrt{k/n_\source}$, we have an overall bound of
  \[
    (\mathrm{I}) \leq \frac{r\norm[2]{\Sigma}^{1/2}}{\sqrt{n_\source T}}\sqrt{kT + kd\log n_\source}.
  \]

  \vspace{2ex}
  \noindent
  \underline{Bounding (II).}
  \vspace{1ex}

  By bounding by the Gaussian complexity,
  \begin{align*}
    (\mathrm{II}) &\leq \frac{1}{n_\source T}\expt{\sup_{\norm[2]{\delta_t} \leq \delta_0}\sum_{t \in [T]}\inprod{z_t, X_t\delta_t}} \lesssim \frac{\delta_0}{\sqrt{n_\source}}\expt{\norm[2]{\frac{1}{\sqrt{n}}X_1^\top z}} \leq \frac{\delta_0}{\sqrt{n_\source}}\sqrt{\tr\Sigma}.
  \end{align*}

  Putting the bounds on (I) and (II) together, we thus have that
  \[
    \frac{1}{T}\mathcal{R}_{n_\source}\left[\Union_{\theta \in \Theta_0}\adaptset_{\theta}^{\constraintset_\source}\right] \lesssim \frac{r\norm[2]{\Sigma}^{1/2}}{\sqrt{n_\source T}}\sqrt{kT + kd\log n_\source} + \frac{\delta_0}{\sqrt{n_\source}}\sqrt{\tr\Sigma}. \qedhere
  \]
\end{proof}


==> results/nonlinear/logistic/logisticTargetRademacher.tex <==
\begin{restatable}[Target Rademacher Bound]{lemma}{logisticTargetRademacher}
  For $\beta \gtrsim r\kappa^{1/2}$, the Rademacher complexity of the feasible set during target time training is bounded by
  \[
    \mathcal{R}_{n_\target}\left(\adaptset_{\theta_0}^{\constraintset_\target}\right) \lesssim r\kappa^{1/2}\norm[2]{\Sigma}^{1/2}\sqrt{\frac{k}{n_\target}} + \frac{\delta_0}{\sqrt{n_\target}}\sqrt{\tr\Sigma}.
  \]
\end{restatable}
\begin{proof}
  We can write the Rademacher complexity as
  \begin{align*}
    \mathcal{R}_{n_\target}\left(\adaptset_{\theta_0}^{\constraintset_\target}\right) = \beta\expt{\sup_{(\Delta, w) \in \constraintset_\target^\beta}\frac{1}{n_\target}\inprod{\epsilon, X[B_0, B_0]w + X\Delta w_0 + X\Delta w}}.
  \end{align*}
  Firstly, by converting to Gaussian complexity and following standard arguments, we can bound the first term as
  \begin{align*}
    \beta\expt{\sup_{\norm[2]{w} \leq r\kappa^{1/2}/\beta}\frac{1}{n_\target}\inprod{z, X[B_0, B_0]w}} &\leq \beta\expt{\sup_{\norm[2]{w} \leq \kappa/\beta}\frac{1}{n_\target}\inprod{[B_0, B_0]^\top X^\top z, w}} \\
      &\leq \frac{r\kappa^{1/2}}{\sqrt{n_\target}}\expt{\norm[2]{B_0^\top \frac{X^\top}{\sqrt{n_\target}} z}} \\
      &\leq r\kappa^{1/2}\norm[2]{\Sigma}^{1/2}\sqrt{\frac{k}{n_\target}}.
  \end{align*}
  For the second term, note that we only need to consider the set of rank-1 matrices of the form $\Delta = v [w_0, -w_0]^\top$, where $\norm[2]{v} \leq \delta_0/\beta\sqrt{2}$.
  As such,
  \[
    \beta\expt{\sup_{\norm[2]{v} \leq \delta_0/\beta\sqrt{2}}\frac{1}{n_\target}\inprod{z, Xv}} \leq \frac{\delta_0}{\sqrt{n_\target}}\sqrt{\expt{\norm[2]{\frac{X}{\sqrt{n_\target}}z}^2}} \lesssim \frac{\delta_0}{\sqrt{n_\target}}\sqrt{\tr\Sigma}.
  \]
  Finally, to bound the Hessian term, note that $\norm[2]{\Delta w} \leq r\kappa^{1/2}\delta_0/\beta^2$. Therefore, by a similar argument to the previous term,
  \[
    \beta\expt{\sup_{(\Delta, w) \in \constraintset_\target}\frac{1}{n_\target}\inprod{\epsilon, X\Delta w}} \leq \frac{\kappa\delta_0}{\beta\sqrt{n_\target}}\sqrt{\tr\Sigma}.
  \]
  Thus, as long as $\beta \geq r\kappa^{1/2}$, we obtain the overall bound of
  \[
    \mathcal{R}_{n_\target}\left(\adaptset_{\theta_0}^{\constraintset_\target}\right) \lesssim r\kappa^{1/2}\norm[2]{\Sigma}^{1/2}\sqrt{\frac{k}{n_\target}} + \frac{\delta_0}{\sqrt{n_\target}}\sqrt{\tr\Sigma}. \qedhere
  \]
\end{proof}


==> results/nonlinear/nn/nnApproximateLinearity.tex <==
\begin{restatable}[Neural network approximate linearity]{lemma}{nnApproximateLinearity}
  Assume that $\gamma^2 \geq 2\kappa$.
  For any $\theta_0 \in \Theta$,
  \[
    \sup_{\delta \in \constraintset_\target}\frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]^2 f^\gamma_{\theta_0 + \delta}(x_i)}^2 \lesssim \gamma^2(L + \mu)^2 \quad \text{and} \quad \frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]f_{\theta_0}^\gamma(x_i)}^2 \lesssim \gamma^2kL^2.
  \]
\end{restatable}
\begin{proof}
  The first bound is a trivial consequence of \lemmaref{lemma:nn-hessian-bound}.
  Meanwhile, we note that the second inequality, the quantity inside the norm is exactly $\beta\rho_{\theta_0}(x)$, and thus the bound follows by \lemmaref{lemma:nn-rep-bound}.
\end{proof}


==> results/nonlinear/nn/nnDiversityCondition.tex <==
\begin{restatable}[Neural network diversity]{lemma}{nnDiversityCondition}
  Assume that $\gamma > \max(\kappa\beta, \sqrt{2\kappa})$.
  The source tasks satisfy a $(1, (L + \mu)^2/\beta^2)$-diversity condition with respect to the target task distribution $\rho$.
\end{restatable}
\begin{proof}
  Observe that we can write the excess risk as
  \[
    \expt{[(\gamma\rho_{B_0, w_0}(x)\delta - \beta\rho_{B^\ast, w_0^\ast}(x)\delta^\ast) + (\gamma\zeta_{B_0, w_0}^{\delta}(x) - \beta\zeta_{B^\ast, w_0^\ast}^{\delta^\ast}(x))]^2}.
  \]
  We proceed to upper bound the averaged best-case target performance, and lower bound the best-case performance averaged over source tasks.

  \vspace{2ex}
  \noindent
  \underline{Upper bounding the expected best-case target performance.}
  \vspace{1ex}

  Fix a $\delta^\ast$.
  Then, since $\gamma^2 > 2\kappa$ guarantees that \lemmaref{lemma:nn-hessian-bound} holds,
  \begin{align*}
    \expt{(f^\beta_{\theta_0 + \delta}(x) - f^\beta_{\theta_0^\ast + \delta^\ast}(x))^2} &\lesssim \expt{(\gamma\rho_{\theta_0}(x)\delta - \rho_{\theta_0^\ast}(x)\delta^\ast)^2} + \expt{(\gamma\zeta_{\theta_0}^{\delta}(x) - \beta\zeta_{\theta_0^\ast}^{\delta^\ast}(x))^2} \\
      &\lesssim \expt{\left(\gamma\rho_{\theta_0}(x)\delta - \beta\rho_{\theta_0^\ast}(x)\delta^\ast\right)^2} + \left[\frac{\kappa}{\gamma}(L + \mu)\right]^2 + \frac{(L + \mu)^2}{\beta^2} \\
      &\lesssim \expt{\left(\gamma\rho_{\theta_0}(x)\delta - \beta\rho_{\theta_0^\ast}(x)\delta^\ast\right)^2} + \frac{(L + \mu)^2}{\beta^2}.
  \end{align*}
  Therefore, by taking the infimum over $\delta \in \constraintset_\target$ and noting that the unconstrained infimum of the right-hand side is feasible by \propref{prop:opt-perf-under-subopt-repr} and the conditioning constraint imposed by $\Theta_0$,
  \[
    \inf_{\delta \in \constraintset_\target^\gamma}\expt{(f^\beta_{\theta_0 + \delta}(x) - f^\beta_{\theta_0^\ast + \delta^\ast}(x))^2} \leq \beta^2\norm[2]{\Lambda(\rho_{\theta_0}, \rho_{\theta_0^\ast})^{1/2}\delta^\ast}^2 + \left(\frac{L + \mu}{\beta}\right)^2
  \]
  Now, by the choice of target task distribution, we can write $\delta^\ast$ as $\Gamma \omega^\ast/\beta$, where we note that $\expt{\omega^\ast(\omega^\ast)^\top} = (1/k)I_{2k}$.
  Thus, by taking expectations, we have that
  \[
    \expt[\delta^\ast \sim \rho]{\inf_{\delta \in \constraintset_\target^\gamma}\expt{(f^\beta_{\theta_0 + \delta}(x) - f^\beta_{\theta_0^\ast + \delta^\ast}(x))^2}} \leq \frac{1}{k}\norm[F]{\Lambda(\rho_{\theta_0}, \rho_{\theta_0^\ast})^{1/2}\Gamma}^2 + \left(\frac{L + \mu}{\beta}\right)^2.
  \]

  \vspace{2ex}
  \noindent
  \underline{Lower bounding the source task-averaged best-case target performance.}
  \vspace{1ex}

  Fix a source task $t \in [T]$.
  By \Cref{cor:quadratic-expectation-lower-bound}, we have the bound
  \begin{align*}
    \beta^2\expt{(\rho_{\theta_0}(x)\delta - \rho_{\theta_0^\ast}(x)\delta_t^\ast)^2} &\lesssim \expt{(f^\beta_{\theta_0 + \delta}(x) - f^\beta_{\theta_t^\ast}(x))^2} + \expt{(\zeta_{\theta_0}^{\delta}(x) - \zeta_{\theta_0^\ast}^{\delta^\ast}(x))^2} \\
      &\lesssim \expt{(f^\beta_{\theta_0 + \delta}(x) - f^\beta_{\theta^\ast}(x))^2} + \left(\frac{L + \mu}{\beta}\right)^2.
  \end{align*}
  Therefore, by taking the infimum on both sides and applying \propref{prop:opt-perf-under-subopt-repr},
  \[
    \norm[2]{\Lambda(\rho_{\theta_0}, \rho_{\theta^\ast})^{1/2}\Gamma\omega_t^\ast}^2 \leq \inf_{\delta \in \constraintset_\source}\expt{(f^\beta_{\theta_0 + \delta}(x) - f^\beta_{\theta^\ast}(x))^2} + \left(\frac{L + \mu}{\beta}\right)^2.
  \]
  By averaging over the set of source tasks,
  \[
    \frac{1}{T}\norm[F]{\Lambda(\rho_{\theta_0}, \rho_{\theta^\ast})^{1/2}\Gamma\Omega}^2 \leq \frac{1}{T}\sum_{t \in [T]}\inf_{\delta \in \constraintset_\source}\expt{(f^\beta_{\theta_0 + \delta}(x) - f^\beta_{\theta^\ast}(x))^2} + \left(\frac{L + \mu}{\beta}\right)^2.
  \]
  Finally, by applying \assumpref{assump:nn-diversity-condition} to lower bound the left-hand side, we find that
  \[
    \frac{1}{k}\norm[F]{\Lambda(\rho_{\theta_0}, \rho_{\theta^\ast})^{1/2}\Gamma}^2 \leq \frac{1}{T}\sum_{t \in [T]}\inf_{\delta \in \constraintset_\source}\expt{(f^\beta_{\theta_0 + \delta}(x) - f^\beta_{\theta^\ast}(x))^2} + \left(\frac{L + \mu}{\beta}\right)^2.
  \]

  \vspace{2ex}
  \noindent
  \underline{Concluding}.
  \vspace{1ex}

  Consequently, by putting the two parts together, we have that
  \begin{align*}
    &\expt[\delta^\ast \sim \rho]{\inf_{\delta \in \constraintset_\target^\gamma}\expt{(f^\beta_{\theta_0 + \delta}(x) - f^\beta_{\theta_0^\ast + \delta^\ast}(x))^2}} \\
      &\qquad \leq \frac{1}{T}\sum_{t \in [T]}\inf_{\delta \in \constraintset_\source}\expt{(f^\beta_{\theta_0 + \delta}(x) - f^\beta_{\theta^\ast}(x))^2} + \left(\frac{L + \mu}{\beta}\right)^2. \qedhere
  \end{align*}
\end{proof}


==> results/nonlinear/nn/nnHessianBound.tex <==
\begin{restatable}[Hessian Bound]{lemma}{nnHessianBound}
  \label{lemma:nn-hessian-bound}
  Fix a matrix $\bar{B} \in \reals^{2k \times d}$ and a vector $\bar{w} \in \reals^{2k}$.
  Assume that all rows of $\bar{B}$ are $2$-norm-bounded, and that $\norm[2]{\bar{w}} \leq 2$.
  Then, for $x \sim p$ almost surely, $\norm[2]{\grad[\theta]^2f^\beta_{(\bar{B}, \bar{w})}(x)} \lesssim \beta(\mu + L)$.
\end{restatable}
\begin{proof}
  Throughout the proof, we will use the fact that $\norm[2]{x} \leq 1$ for $x \sim p$ almost surely.
  By definition,
  \[
    \norm[2]{\grad[\theta]^2f^\beta_{(\bar{B}, \bar{w})}(x)} = \sup_{\norm[F]{\Delta}^2 + \norm[2]{w}^2 \leq 1}\beta\abs{\sum_{i \in [2k]}\bar{w}_i\sigma''(\bar{B}_i^\top x)\inprod{\Delta_i, x}^2 + 2\sum_{i \in [2k]}w_i\sigma'(\bar{B}_i^\top x)\inprod{\Delta_i, x}}
  \]
  To bound the first term, observe that by applying H\"older's inequality,
  \begin{align*}
    \sum_{i \in [2k]}\bar{w}_i\sigma''(\bar{B}_i^\top x)\inprod{\Delta_i, x}^2 &\leq \left(\sup_{i \in [2k]}\abs{w_i\sigma''(\bar{B_i}^\top x)}\right)\sum_{i \in [2k]}\inprod{\Delta_i, x}^2 \\
    &= \left(\sup_{i \in [2k]}\abs{\bar{w_i}\sigma''(\bar{B_i}^\top x)}\right)\norm[2]{\Delta x}^2 \leq 2\mu.
  \end{align*}
  To bound the second term, we apply Cauchy-Schwarz, from which we see that
  \begin{align*}
    2\sum_{i \in [2k]}w_i\sigma'(\bar{B}_i^\top x)\inprod{\Delta_i, x} &\leq 2\left(\sum_{i \in 2k}\left[w_i\sigma'(\bar{B_i}^\top x)\right]^2\right)^{1/2}\norm[2]{\Delta x} \\
      &\leq 2L\norm[2]{w}\norm[2]{\Delta x} \leq 2L.
  \end{align*}
  Altogether, we thus have that almost surely for $x \sim p$,
  \[
    \norm[2]{\grad[\theta]^2f^\beta_{(\bar{B}, \bar{w})}(x)} \lesssim \beta(\mu + L). \qedhere
  \]
\end{proof}


==> results/nonlinear/nn/nnLossAssumpValidation.tex <==
\begin{restatable}[Validating Loss Assumptions]{lemma}{nnLossAssumpValidation}
  Assume that $\gamma^2 \geq 2\kappa$.
  Define the quantities
  \[
    \alpha_1 \defas L\sqrt{k} + \frac{\mu + L}{\beta} \quad \text{and} \quad \alpha_2 \defas \kappa^{1/2}L\sqrt{k} + \frac{\kappa}{\gamma}\left(\mu + L\right).
  \]
  Then, during both source and target training time, $\abs{\ell(0, y)} \leq \alpha_1^2$ for any $y$, and $\ell(\cdot, y)$ is $\alpha_1$-Lipschitz during source training time and $\alpha_2$-Lipschitz during target training time for any $y$, all up to universal constants.
\end{restatable}
\begin{proof}
  For the squared error loss, $\ell(0, y) = y^2$ and $\grad[\hat{y}]\ell(\hat{y}, y) = 2(\hat{y} - y)$ for any $y$.
  Therefore, since the additive noise is $O(1)$ bounded, the claims hold as long as we can prove a bound on the predictions of any feasible predictor.

  We first consider bounding the Lipschitz constant during source-time training.
  That is, we need to provide a uniform bound on $x \mapsto \beta\rho_{\theta_0}(x)^\top\delta + \beta\zeta_{\theta_0}^{\delta}(x)$ for $\theta_0 \in \Theta_0$, $\delta \in \constraintset_\source$, and $x$ in the support of $p$.
  To this end, we apply the bounds in \Cref{corollary:nn-remainder-bound} and \lemmaref{lemma:nn-rep-bound}, from which we obtain
  \[
    \abs{\beta\rho_{\theta_0}(x)^\top\delta + \beta\zeta_{\theta_0}^\delta(x)} \lesssim L\sqrt{k} + \frac{\mu + L}{\beta} \asdef \alpha_1.
  \]
  By applying a similar argument for target-time training, we find that
  \[
    \abs{\gamma\rho_{\theta_0}(x)^\top\delta + \gamma\zeta_{\theta_0}^\delta(x)} \lesssim \kappa^{1/2}L\sqrt{k} + \frac{\kappa}{\gamma}\left(\mu + L\right) \asdef \alpha_2.
  \]

  We thus can conclude that during both source and target training time, $\abs{\ell(0, y)} \leq \alpha_1^2$ for any $y$, and that $\ell(\cdot, y)$ is $\alpha_1$-Lipschitz during source training time and $\alpha_2$-Lipschitz during target training time for any feasible $y$.
\end{proof}


==> results/nonlinear/nn/nnPerformanceBound.tex <==
\begin{restatable}[Neural net performance bound]{theorem}{nnPerformanceBound}
  Assume that \Cref{assump:nn-activation-assump,assump:nn-init-assump,assump:nn-diversity-condition} hold.
  Then, if $n_\source \geq n_\target$, there exists a training parameter setting (see \secref{sec:case-study-proofs}) such that with probability at least $1 - \delta$, the iterates $(\theta_t)$ satisfy
  \IfAppendix{
    \[
      \expt[f^\ast \sim \rho]{\min_t\meanloss_\infty^{f^\ast}(f_{\theta_t}) - \meanloss_\infty^{f^\ast}(f_{\theta^\ast})} \lesssim \kappa L^2\frac{k}{\sqrt{n_\target}} + L(L + \mu)\frac{k^{3/2}}{\sqrt{n_\source T}} + \left(\frac{\mu + L}{\beta}\right)L\sqrt{k}.
    \]
  }{
    \begin{align*}
      &\expt[f^\ast \sim \rho]{\min_t\meanloss_\infty^{f^\ast}(f_{\theta_t}) - \meanloss_\infty^{f^\ast}(f_{\theta^\ast})} \lesssim \kappa L^2\frac{k}{\sqrt{n_\target}} + L(L + \mu)\frac{k^{3/2}}{\sqrt{n_\source T}} + \left(\frac{\mu + L}{\beta}\right)L\sqrt{k}.
    \end{align*}
  }
\end{restatable}
\begin{proof}
  By incorporating previous bounds and invoking \thmref{thm:general-performance-bound}, we have that for large enough $\gamma$,
  \begin{align*}
    &\expt[f^\ast \sim \rho]{\min_t\meanloss_\infty^{f^\ast}(f_{\theta_t}(x)) - \meanloss_\infty^{f^\ast}(\theta^\ast)} \\
      &\qquad \lesssim \sqrt{\frac{k\kappa(L + \mu)^2}{T_\pgd}} + \kappa L^2\frac{k}{\sqrt{n_\target}} + L(L + \mu)\frac{k^{3/2}}{\sqrt{n_\source T}} + \left(\frac{\mu + L}{\beta}\right)L\sqrt{k}.
  \end{align*}
  Therefore, by running enough projected gradient descent iterations so that the first term matches $kL^2k/\sqrt{n_\target}$, we obtain the desired bound.
\end{proof}


==> results/nonlinear/nn/nnRepresentationBound.tex <==
\begin{restatable}[Representation Norm Bound]{lemma}{nnRepresentationBound}
  \label{lemma:nn-rep-bound}
  For $x \sim p$, $\norm[2]{\rho_{\theta_0}(x)} \leq 2L\sqrt{k}$ almost surely for any $\theta_0 = (B_0, w_0) \in \Theta_0$.
\end{restatable}
\begin{proof}
  Recall from definitions that $\norm[2]{\rho_{\theta_0}(x)}^2 = \norm[2]{\phi_{B_0}(x)}^2 + \norm[F]{\psi_{\theta_0}(x)}^2$.
  To bound the activation features, since $\sigma(0) = 0$ and $\abs{\sigma'(x)} \leq L$ for $x \in [-1, 1]$,
  \[
    \norm[2]{\phi_{B_0}(x)}^2 = 2k\max_{i \in [2k]}\abs{\sigma(B_{0, i}^\top x)}^2 \leq 2k\max_{i \in [2k]}\abs{\int_{0}^{B_{0, i}^\top x}\sigma'(z) \ \diff{z}}^2 \leq 2kL^2.
  \]
  To bound the gradient features, we once again use the boundedness of $\sigma'$ to obtain
  \begin{align*}
    \norm[F]{\psi_{\theta_0}(x)}^2 &= \norm[F]{w_0^{\mathrm{diag}}\sigma'(B_0^\top x)x^\top}^2 = \norm[2]{w_0^{\mathrm{diag}}\sigma'(B_0^\top x)}^2\norm[2]{x}^2 = \norm[2]{\sigma'(B_0^\top x)}^2\norm[2]{x}^2 \leq 2kL^2.
  \end{align*}
  Putting the bounds together, we obtain the desired overall bound.
\end{proof}


==> results/nonlinear/nn/nnSourceRademacher.tex <==
\begin{restatable}[Source Rademacher Bound]{lemma}{nnSourceRademacher}
  We have the following bound on the Rademacher complexity:
  \[
    \frac{1}{T}\mathcal{R}_{n_\source}\left[\Union_{\theta \in \Theta_0}\adaptset_{\theta}^{\constraintset_\source}\right] \lesssim \frac{kL}{(n_\source T)^2} + \left[(L + \mu)\frac{k}{\sqrt{n_\source T}} + L\sqrt{\frac{k}{n_\source}}\right]\log(n_\source T) + \frac{\mu + L}{\beta}
  \]
\end{restatable}
\begin{proof}
  We first consider bounding the empirical Rademacher complexity for a fixed set of inputs $(x_{i, t})$, after which we obtain the desired result by taking expectations over the sampled inputs.
  Expanding the definition, we have that
  \begin{align*}
    &\frac{1}{T}\mathcal{R}_{n_\source}\left[\Union_{\theta \in \Theta_0}\adaptset_{\theta}^{\constraintset_\source}\right] \\
      &\qquad = \frac{1}{nT}\expt{\sup_{\substack{(B_0, w_0) \in \Theta_0 \\ (\Delta_t, w_t) \in \constraintset_\source}}\abs{\sum_{\substack{i \in [n_\source] \\ t \in [T]}}\epsilon_{i, t}\left[w_t^\top \phi(B^\top x_{i, t}) + \inprod{\Delta_t, \psi_{B}(x_{i, t})} + \zeta_{B, w_0}^{\Delta_t, w_t}(x_{i, t})\right]}} \\
      &\qquad \leq \frac{1}{T}\mathcal{R}_{n_\source}(\mathcal{F}_\Phi^{\otimes T} \comp \Phi) + \frac{1}{T}\mathcal{R}_{n_\source}(\mathcal{F}_\Psi^{\otimes T} \comp \Psi) + \frac{\mu + L}{\beta},
  \end{align*}
  where
  \begin{align*}
    \mathcal{F}_\Phi &\defas \set{z \mapsto \beta\inprod{w, z} \suchthat \norm[2]{w} \leq 1/\beta} \\
    \mathcal{F}_\Psi &\defas \set{Z \mapsto \beta\inprod{\Delta, Z} \suchthat \norm[F]{\Delta} \leq 1/\beta} \\
    \Phi &\defas \set{\phi_{B} \suchthat (\exists w) \ (B, w) \in \Theta_0} \\
    \Psi &\defas \set{\psi_{B, w} \suchthat (B, w) \in \Theta_0}.
  \end{align*}
  We proceed to bound the two complexity terms by noting that for any function class $\mathcal{F}$, $\mathcal{R}_{n_\source}(\mathcal{F}) \lesssim \mathcal{G}_{n_\source}(\mathcal{F})$, and making use of the Gaussian complexity chain rule from \propref{prop:gauss-comp-chain-rule}.
  First, note that for a fixed set of latent vectors $z_1, \dots, z_{n_\source}$,
  \[
    \mathcal{G}_Z(\mathcal{F}_\Phi) = \frac{1}{n_\source}\expt{\sup_{\norm[2]{w} \leq 1}\abs{\inprod{z, Zw}}} \leq \frac{1}{n_\source}\sqrt{\tr{ZZ^\top}} = \frac{1}{n_\source}\sqrt{\sum_{i \in [n_\source]}\norm[2]{z_i}^2\vphantom{\sum^T}}.
  \]
  Then, applying the representation norm bound \lemmaref{lemma:nn-rep-bound} to the latents,
  \[
    \expt{\max_{Z \in \mathcal{Z}}\mathcal{G}_Z(\mathcal{F}_\Phi)} \leq L\sqrt{\frac{k}{n_\source}}.
  \]
  Similarly, for a fixed set of latent matrices $Z_1, \dots, Z_{n_\source}$
  \[
    \mathcal{G}_Z(\mathcal{F}_\Psi) \leq \frac{1}{n_\source}\sqrt{\sum_{i \in n_\source}\norm[F]{Z_i}^2\vphantom{\sum^T}} \implies \expt{\max_{Z \in \mathcal{Z}}\mathcal{G}_Z(\mathcal{F}_\Psi)} \leq L\sqrt{\frac{k}{n_\source}},
  \]
  where we once again used the representation bound from \lemmaref{lemma:nn-rep-bound}.

  Finally, we bound the complexity of the classes $\Phi$ and $\Psi$.
  Firstly, we have
  \begin{align*}
    \frac{1}{T}\mathcal{G}_{n_\source}(\Phi) &= \frac{1}{n_\source T}\expt{\sup_{(B_0, w_0) \in \Theta_0}\abs{\sum_{r \in [2k]}\sum_{i \in [n_\source]}\sum_{t \in [T]}z_{r, i, t}\sigma(B_r^\top x_{i, t})}} \\
      &\leq \frac{2k}{n_\source T}\expt{\sup_{\norm[2]{b} \leq 1} \abs{\sum_{i \in [n_\source]}\sum_{t \in [T]}z_{i, t}\sigma(b^\top x_{i, t})}} \\
      &\lesssim \frac{kL}{n_\source T}\expt{\norm[2]{\sum_{i \in [n_\source T]}z_ix_i}} \leq \frac{kL}{n_\source T}\sqrt{\sum_{i \in [n_\source T]}\norm[2]{x_i}^2\vphantom{\sum^T}} \leq \frac{kL}{\sqrt{n_\source T}}.
  \end{align*}
  where the second inequality makes use of the Gaussian contraction result in \citet[Corollary 3.17]{ledoux1991probability}.
  Note that we reindex at the third line, which is made possible by the fact that the source tasks have the same input distributions.
  Secondly,
  \begin{align*}
    \frac{1}{T}\mathcal{G}_{n_\source}(\Psi) &= \frac{1}{n_\source T}\expt{\sup_{(B_0, w_0) \in \Theta_0}\abs{\sum_{r \in [2k]}\sum_{i \in [n_\source]}\sum_{t \in [T]}\sigma'(B_r^\top x_{i, t})\inprod{x_{i, t}, z_{r, i, t}}}} \\
      &= \frac{1}{n_\source T}\expt{\sup_{(B_0, w_0) \in \Theta_0}\abs{\sum_{r \in [2k]}\sum_{i \in [n_\source]}\sum_{t \in [T]}[\sigma'(B_r^\top x_{i, t}) - \sigma'(0)]\inprod{x_{i, t}, z_{r, i, t}}}} + \frac{L}{\sqrt{n_\source T}} \\
      &= \frac{2k}{n_\source T}\expt{\sup_{\norm[2]{b} \leq 1}\abs{\sum_{i \in [n_\source]}\sum_{t \in [T]}\left[\sigma'(b^\top x_{i, t}) - \sigma'(0)\right]\inprod{x_{i, t}, z_{r, i, t}}}} + \frac{L}{\sqrt{n_\source T}} \\
      &\lesssim \frac{k\mu}{n_\source T}\expt{\norm[2]{\sum_{i \in [n_\source T]}\inprod{x_{i, t}, z_{i, t}}x_{i, t}}} + \frac{L}{\sqrt{n_\source T}} \leq \frac{k\mu}{n_\source T}\sqrt{\sum_{i \in [n_\source T]}\norm[2]{x_i}^4\vphantom{\sum^T}} + \frac{L}{\sqrt{n_\source T}} \\
      &\leq \frac{k\mu}{\sqrt{n_\source T}} + \frac{L}{\sqrt{n_\source T}},
  \end{align*}
  following the same reasoning as before.
  Therefore, by applying \propref{prop:gauss-comp-chain-rule}, we obtain the bound
  \[
    \frac{1}{T}\mathcal{R}_{n_\source}\left[\Union_{\theta \in \Theta_0}\adaptset_{\theta}^{\constraintset_\source}\right] \lesssim \frac{kL}{(n_\source T)^2} + \left[(L + \mu)\frac{k}{\sqrt{n_\source T}} + L\sqrt{\frac{k}{n_\source}}\right]\log(n_\source T) + \frac{\mu + L}{\beta}. \qedhere
  \]
\end{proof}


==> results/nonlinear/nn/nnTargetRademacher.tex <==
\begin{restatable}[Target Rademacher bound]{lemma}{nnTargetRademacher}
  We have the following Rademacher complexity bound:
  \[
    \mathcal{R}_{n_\target}(\adaptset_{\theta_0}^{\constraintset_\target^\gamma}) \lesssim L\sqrt{\kappa}\sqrt{\frac{k}{n_\target}} + \frac{\kappa}{\gamma}(L + \mu). \qedhere
  \]
\end{restatable}
\begin{proof}
  Following definitions, we have that
  \begin{align*}
    \mathcal{R}_{n_\target}(\adaptset_{\theta_0}^{\constraintset_\target^\gamma}) &= \frac{\gamma}{n_\target}\expt{\sup_{\delta \in \constraintset_\target^\gamma}\abs{\inprod{\epsilon, \rho(X)\delta + \zeta_{\theta_0}^{\delta}(X)}}} \leq \frac{\gamma}{n_\target}\expt{\sup_{\delta \in \constraintset_\target^\gamma}\abs{\inprod{\epsilon, \rho(X)\delta}}} + \frac{\kappa}{\gamma}(L + \mu) \\
      &= \frac{\sqrt{\kappa}}{n_\target}\expt{\norm[2]{\rho(X)^\top \epsilon}} + \frac{\kappa}{\gamma}(L + \mu) \leq \frac{\sqrt{\kappa}}{n_\target}\sqrt{\expt{\norm[2]{\rho(X)^\top \epsilon}^2}} + \frac{\kappa}{\gamma}(L + \mu) \\
      &\leq L\sqrt{\kappa}\sqrt{\frac{k}{n_\target}} + \frac{\kappa}{\gamma}(L + \mu),
  \end{align*}
  where the final inequality uses the bound on the representation given in \lemmaref{lemma:nn-rep-bound}.
\end{proof}


==> results/nonlinear/perf/approximateConvexity.tex <==
\begin{restatable}[Approximate convexity in $\mathcal{B}$]{lemma}{approximateConvexity}
  \label{lemma:approximate-convexity}
  Let $\theta_1, \theta_2 \in \mathcal{B}$.
  Then,
  \[
    \inprod{\grad[\theta]\meanloss(\theta_1), \theta_2 - \theta_1} \leq \meanloss(\theta_2) - \meanloss(\theta_1) + 4\gamma\delta_0^2\sqrt{\frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]^2g_{\bar\theta}(x_i)}^2\vphantom{\sum^T}}.
  \]
\end{restatable}
\begin{proof}
  Note that we can view $\meanloss$ as the composition of functions $\bar{\meanloss}: \reals^{n_\target} \to \reals$ and $g_{\cdot}(X) : \Theta \to \reals^{n_\target}$, where we define
  \[
    \bar{\meanloss}(g_1, \dots, g_n) \defas \frac{1}{n_\target}\sum_{i \in [n_\target]}\ell(g_i, y_i) \quad \text{and} \quad g_{\theta}(X) = [g_\theta(x_1), \dots, g_\theta(x_n)]^\top.
  \]
  Since $\ell$ is convex in its first argument, $\bar{\mathcal{L}}$ is convex.
  Thus,
  \[
    \meanloss(\theta_2) - \meanloss(\theta_1) \geq \inprod{\grad[(g_1, \dots, g_n)]{\bar{\meanloss}(g_{\theta_1}(X))}, g_{\theta_2}(X) - g_{\theta_1}(X)}.
  \]
  Furthermore, by the chain rule,
  \[
    \inprod{\grad[\theta]\meanloss(\theta_1), \theta_2 - \theta_1} = \inprod{\grad[(g_1, \dots, g_n)]\bar{\meanloss}(g_{\theta_1}(X)), \grad[\theta]g_{\theta_1}(X)(\theta_2 - \theta_1)}.
  \]
  Putting the two statements together and applying Cauchy-Schwarz,
  \begin{align*}
    &\meanloss(\theta_2) - \meanloss(\theta_1) - \inprod{\grad[\theta]\meanloss(\theta_1), \theta_2 - \theta_1} \\
      &\quad \geq \inprod{\grad[(g_1, \dots, g_n)]{\bar{\meanloss}(g_{\theta_1}(X))}, g_{\theta_2}(X) - g_{\theta_1}(X) - \grad[\theta]g_{\theta_1}(X)(\theta_2 - \theta_1)} \\
      &\quad \geq -\norm[2]{\grad[(g_1, \dots, g_n)]{\bar{\meanloss}(g_{\theta_1}(X))}}\norm[2]{g_{\theta_2}(X) - g_{\theta_1}(X) - \grad[\theta]g_{\theta_1}(X)(\theta_2 - \theta_1)} \\
      &\quad \geq -\frac{1}{\sqrt{n_\target}}\norm[2]{g_{\theta_2}(X) - g_{\theta_1}(X) - \grad[\theta]g_{\theta_1}(X)(\theta_2 - \theta_1)}
  \end{align*}
  Now, by Taylor's theorem, there exists $\bar\theta = \lambda\theta_1 + (1 - \lambda)\theta_2$ such that
  \[
    g_{\theta_2}(X) - g_{\theta_1}(X) - \grad[\theta]g_{\theta_1}(X)(\theta_2 - \theta_1) = [(\theta_2 - \theta_1)^\top\grad[\theta]^2g_{\bar\theta}(x_i)(\theta_2 - \theta_1)]_{i \in [n_\target]}.
  \]
  Consequently, by rearranging,
  \begin{align*}
    \inprod{\grad[\theta]\meanloss(\theta_1), \theta_2 - \theta_1} &\leq \meanloss(\theta_2) - \meanloss(\theta_1) + \frac{1}{\sqrt{n_\target}}\sqrt{\sum_{i \in [n_\target]}[(\theta_2 - \theta_1)^\top\grad[\theta]^2g_{\bar\theta}(x_i)(\theta_2 - \theta_1)]^2\vphantom{\sum^T}} \\
      &\leq \meanloss(\theta_2) - \meanloss(\theta_1) + \norm[2]{\theta_2 - \theta_1}^2\sqrt{\frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]^2g_{\bar\theta}(x_i)}^2\vphantom{\sum^T}} \\
      &\leq \meanloss(\theta_2) - \meanloss(\theta_1) + 4\gamma\delta_0^2\sqrt{\frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]^2g_{\bar\theta}(x_i)}^2\vphantom{\sum^T}}. \qedhere
  \end{align*}
\end{proof}


==> results/nonlinear/perf/genPerformanceBound.tex <==
\begin{restatable}[General Performance Bound]{theorem}{genPerformanceBound}
  \label{thm:general-performance-bound}
  Assume that \Cref{assump:loss-fn-assumptions,assump:nu-eps-diversity-def,assump:adapt-approx-linearity,assump:target-adapt-norm-bound} all hold.
  Consider a learner following the training procedure outlined in \secref{sec:gen-train-proc}, and let $(\theta_t)$ be the set of iterates generated by PGD with appropriately chosen step size $\eta$ \IfAppendix{}{(specified in \secref{sec:gen-perf-proofs})}.
  Then, with probability at least $1 - \delta$ over the random draw of samples,
  \begin{align*}
    \expt[g^\ast \distas \rho]{\min_t\meanloss^{g^\ast}_\infty(\theta_t) - \meanloss_\infty^{g^\ast}(\theta^\ast + \delta^\ast)} &\lesssim \underbrace{\beta R^2 + R\sqrt{\frac{L^2 + \beta^2R^2}{T_{\mathrm{PGD}}}}}_{\epsilon_{\mathrm{OPT}}} + \underbrace{\frac{1}{\delta}\mathcal{R}_{n_\target}\left(\adaptset_{\theta_0}^{\constraintset_\target}\right) + \frac{B}{\delta\sqrt{n_\target}}}_{\epsilon_{\mathrm{EST}}} \\
      &\qquad + \underbrace{\frac{1}{\nu}\left\{\frac{1}{\delta T}\mathcal{R}_{n_\source}\left[\Union_{\theta \in \Theta_0}\left(\adaptset_{\theta}^{\constraintset_\source}\right)^{\otimes T}\right] + \frac{B}{\delta\sqrt{n_\source T}}\right\} + \epsilon}_{\epsilon_{\mathrm{REPR}}}.
  \end{align*}
  Note that the $\mathcal{R}_{n_\target}$ complexity term samples from $p$, while the $\mathcal{R}_{n_\source}$ complexity term samples from $p^{\otimes T}$, i.e. each draw is $T$ i.i.d. draws from $p$, concatenated.
\end{restatable}
\begin{proof}
  We instantiate the high-probability events in \Cref{lemma:nonlin-src-train-bound,lemma:nonlin-targ-train-bound} both with failure probability $\delta/2$, which simultaneously occur with probability at least $1 - \delta$ via a union-bound.
  Consequently, we have the bounds
  \begin{align*}
    \frac{1}{T}\sum_{t \in [T]}\inf_{g_t \in \adaptset_\theta^{\constraintset_\source}}\meanloss_{\infty}^{g_t^\ast}(g_t) - \meanloss_{\infty}^{g_t^\ast}(g_t^\ast) &\lesssim \frac{1}{\delta T}\mathcal{R}_{n_\source}\left[\Union_{\theta \in \Theta_0}\left(\adaptset_\theta^{\constraintset_\source}\right)^{\otimes T}\right] + \frac{B}{\delta\sqrt{n_\source T}} \\
    \sup_{\substack{g^\ast \in \mathcal{S} \\ g \in \adaptset_{\theta_0}^{\constraintset_\target}}}\abs{\meanloss^{g^\ast}(g) - \meanloss^{g^\ast}_\infty(g)} &\leq \frac{1}{\delta}\mathcal{R}_{n_\target}\left(\adaptset_{\theta_0}^{\constraintset_\target}\right) + \frac{B}{\delta\sqrt{n_\target}}
  \end{align*}

  Given $g^\ast$, let $\bar{g}$ be the population risk minimizer in $\adaptset_{\theta_0}^{\constraintset_\target}$.
  Througout this proof, we omit $g^\ast$ when writing $\meanloss$ and $\meanloss_\infty$ whenever it is understood.
  Then, by \lemmaref{lemma:target-opt-perf}, projected gradient descent always finds an iterate $\tilde g$ such that
  \begin{equation}
    \label{eqn-int:nonlin-opt-bound}
    \meanloss(\tilde g) - \meanloss(\bar g) \lesssim \beta R^2 + R\sqrt{\frac{L^2 + \beta^2 R^2}{T_{\mathrm{PGD}}}},
  \end{equation}
  independent of $g^\ast$.
  Furthermore, note that $\min_t\meanloss_\infty(g_t) - \meanloss_\infty(g^\ast) \leq \meanloss_\infty(\tilde g) - \meanloss_\infty(g^\ast)$.
  We thus proceed to decompose the risk as
  \begin{align*}
    \meanloss_\infty(\tilde g) - \meanloss_\infty(g^\ast) &\lesssim \underbrace{\meanloss_\infty(\tilde g) - \meanloss(\tilde g)}_{\asdef T_1} + \underbrace{\meanloss(\tilde g) - \meanloss(\bar g)}_{\asdef T_2} \\
      &\quad + \underbrace{\meanloss(\bar g) - \meanloss_\infty(\bar g)}_{\asdef T_3} + \underbrace{\meanloss_\infty(\bar g) - \meanloss_\infty(g^\ast)}_{\asdef T_4}.
  \end{align*}
  We now bound the terms $T_1, \dots, T_4$ individually.
  As a result of uniform convergence as guaranteed by \lemmaref{lemma:nonlin-targ-train-bound},
  \[
    T_1, T_3 \leq \sup_{\substack{g^\ast \in \mathcal{S} \\ g \in \adaptset_{\theta_0}^{\constraintset_\target}}}\abs{\meanloss^{g^\ast}(g) - \meanloss^{g^\ast}_\infty(g)} \lesssim \frac{1}{\delta}\mathcal{R}_{n_\target}\left(\adaptset_{\theta_0}^{\constraintset_\target}\right) + \frac{B}{\delta\sqrt{n_\target}},
  \]
  where $\mathcal{S}$ is the support of the target task distribution $\rho$.
  Furthermore, we have demonstrated a bound on $T_2$ in \eqnref{eqn-int:nonlin-opt-bound}.
  Finally, by applying the $(\nu, \epsilon)$-diversity condition as guaranteed by \assumpref{assump:nu-eps-diversity-def},
  \begin{align*}
    \expt[g^\ast \distas \rho]{T_4} &= \expt[g^\ast \distas \rho]{\inf_{g \in \adaptset_{\theta_0}^{\constraintset_\target}}\meanloss_\infty^{g^\ast}(g) - \meanloss_\infty^{g^\ast}(g^\ast)} \\
      &\leq \frac{1}{\nu}\left[\frac{1}{T}\sum_{t \in [T]}\inf_{g_t \in \adaptset_\theta^{\constraintset_\source}}\meanloss_{\infty}^{g_t^\ast}(g_t) - \meanloss_{\infty}^{g_t^\ast}(g_t^\ast)\right] + \epsilon \\
      &\leq \frac{1}{\nu}\left\{\frac{1}{\delta T}\mathcal{R}_{n_\source}\left[\Union_{\theta \in \Theta_0}\left(\adaptset_{\theta}^{\constraintset_\source}\right)^{\otimes T}\right] + \frac{B}{\delta\sqrt{n_\source T}}\right\} + \epsilon.
  \end{align*}
  Taking the expectation with respect to $g^\ast \distas \rho$ and putting all of these bounds together, we thus have that
  \begin{align*}
    &\expt[g^\ast \distas \rho]{\meanloss^{g^\ast}_\infty(\theta_t) - \meanloss_\infty^{g^\ast}(\theta^\ast + \delta^\ast)} \\
      &\qquad \lesssim \beta R^2 + R\sqrt{\frac{L^2 + \beta^2R^2}{T_{\mathrm{PGD}}}} + \frac{1}{\delta}\mathcal{R}_{n_\target}\left(\adaptset_{\theta_0}^{\constraintset_\target}\right) + \frac{B}{\delta\sqrt{n_\target}} \\
      &\qquad\quad + \frac{1}{\nu}\left\{\frac{1}{\delta T}\mathcal{R}_{n_\source}\left[\Union_{\theta \in \Theta_0}\left(\adaptset_{\theta}^{\constraintset_\source}\right)^{\otimes T}\right] + \frac{B}{\delta\sqrt{n_\source T}}\right\} + \epsilon. \qedhere
  \end{align*}
\end{proof}


==> results/nonlinear/perf/gradientBound.tex <==
\begin{restatable}[Gradient bound in $\mathcal{B}$]{lemma}{gradientBound}
  \label{lemma:gradient-bound}
  For any $\theta \in \mathcal{B}$, we have that
  \[
    \norm[2]{\grad[\theta]\meanloss(\theta)}^2 \lesssim \frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]g_{\theta_0}(x_i)}^2 + \gamma\delta_0^2\int_{0}^{1}\frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]^2g_{\alpha\theta + (1 - \alpha)\theta_0}(x_i)}^2 \ \diff{\alpha}
  \]
\end{restatable}
\begin{proof}
  By Jensen's inequality and the fact that $\ell(\cdot, y)$ is $1$-Lipschitz for any $y$,
  \begin{align*}
    \norm[2]{\grad[\theta]\meanloss(\theta)}^2 &= \norm[2]{\frac{1}{n}\sum_{i \in [n_\target]}\grad[\theta]\ell(g_{\theta}(x_i), y_i)}^2 \leq \frac{1}{n}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]\ell(g_{\theta}(x_i), y_i)}^2 \\
      &= \frac{1}{n_\target}\sum_{i \in [n_\target]}\abs{\frac{\partial}{\partial g}\ell(g_{\theta}(x_i), y_i)}^2\norm[2]{\grad[\theta]{g_\theta(x_i)}}^2 \\
      &\leq \frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]{g_\theta(x_i)}}^2
  \end{align*}
  Now, by integrating, we have that for any fixed $i \in [n_\target]$,
  \[
    \grad[\theta]g_\theta(x_i) = \grad[\theta]g_{\theta_0}(x_i) + \left[\int_{0}^{1}\grad[\theta]^2g_{\alpha\theta + (1 - \alpha)\theta_0}(x_i) \ \diff{\alpha}\right](\theta - \theta_0).
  \]
  Therefore,
  \begin{align*}
    \norm[2]{\grad[\theta]\meanloss(\theta)}^2 &\lesssim \frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]g_{\theta_0}(x_i)}^2 + \norm[2]{\int_{0}^{1}\grad[\theta]^2g_{\alpha\theta + (1 - \alpha)\theta_0}(x_i) \ \diff{\alpha}}^2\norm[2]{\theta - \theta_0}^2 \\
      &\leq \frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]g_{\theta_0}(x_i)}^2 + \norm[2]{\theta - \theta_0}^2\int_{0}^{1}\frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]^2g_{\alpha\theta + (1 - \alpha)\theta_0}(x_i)}^2 \ \diff{\alpha} \\
      &\leq \frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]g_{\theta_0}(x_i)}^2 + \gamma\delta_0^2\int_{0}^{1}\frac{1}{n_\target}\sum_{i \in [n_\target]}\norm[2]{\grad[\theta]^2g_{\alpha\theta + (1 - \alpha)\theta_0}(x_i)}^2 \ \diff{\alpha}. \qedhere
  \end{align*}
\end{proof}


==> results/nonlinear/perf/pgdPerformance.tex <==
\begin{restatable}[Bound on PGD performance]{lemma}{pgdPerformance}
  \label{lemma:pgd-performance-bound}
  Assume we run projected gradient descent for $T_\pgd$ iterations with step size $\eta$ given by
  \[
    \eta = \frac{1}{\sqrt{T_\pgd}}\left(\frac{2\gamma\delta_0^2}{L^2 + \beta^2\gamma\delta_0^2}\right)^{1/2}.
  \]
  Let $(\theta_0 + \delta_t)_{t \in [T]}$ denote the sequence of PGD iterates obtained, where $\delta_0 = 0$.
  Then, for any $\norm{\delta} \leq \delta_0$, there exists an iterate $\theta_0 + \delta_t$, $t \in \set{0, \dots, T - 1}$ that satisfies
  \[
    \meanloss(\theta_0 + \delta_t) - \meanloss(\theta_0 + \delta) \lesssim \beta\gamma\delta_0^2 + \sqrt{\frac{\gamma\delta_0^2(L^2 + \beta^2\gamma\delta_0^2)}{T_\pgd}}.
  \]
\end{restatable}
\begin{proof}
  Fix a $\delta$ with $\norm{\delta} \leq \delta_0$, and define $r_t \defas \norm[2]{\delta_t - \delta}$.
  Then, for any $t \in [T_\pgd]$,
  \begin{align*}
    r_{t + 1}^2 &= \norm[2]{\delta_t - \delta}^2 = \norm[2]{(\theta_0 + \delta_{t + 1}) - (\theta_0 + \delta)}^2 \\
      &\leq \norm[2]{\delta_t - \eta\grad[\theta]\meanloss(\theta_0 + \delta_t) - \delta}^2 \\
      &= r_t^2 + 2\eta\inprod{\grad[\theta]\meanloss(\theta_0 + \delta_t), (\theta_0 + \delta) - (\theta_0 + \delta_t)} + \eta^2\norm[2]{\grad[\theta]\meanloss(\theta_0 + \delta_t)}^2 \\
      &\leq r_t^2 + 2\eta\left[\meanloss(\theta_0 + \delta) - \meanloss(\theta_0 + \delta_t) + 4\beta\gamma\delta_0^2\right] + \eta^2\left[L^2 + \beta^2\gamma\delta_0^2\right],
  \end{align*}
  where the first inequality follows from the fact that projections onto convex sets is nonexpansive.
  Via telescoping, we thus have that
  \[
    r_{T_\pgd}^2 \leq r_0^2 + 2\eta\left[\sum_{t = 0}^{T_\pgd - 1}\meanloss(\theta_0 + \delta) - \meanloss(\theta_0 + \delta_t)\right] + 8\eta T_\pgd\beta\gamma\delta_0^2 + \eta^2T_\pgd[L^2 + \beta^2\gamma\delta_0^2],
  \]
  or by rearranging,
  \begin{align*}
    \frac{r_0^2 - r_{T_\pgd}^2}{2\eta T_\pgd} + 4\beta\gamma\delta_0^2 + \eta\left[L^2 + \beta^2\gamma\delta_0^2\right] &\geq \frac{1}{T_\pgd}\sum_{t = 0}^{T_\pgd - 1}\meanloss(\theta_0 + \delta_t) - \meanloss(\theta_0 + \delta) \\
      &\geq \min_{t = 0, \dots, T_\pgd - 1}\meanloss(\theta_0 + \delta_t) - \meanloss(\theta_0 + \delta).
  \end{align*}
  Now, using the choice of step size, observe that
  \begin{align*}
    \frac{r_0^2 - r_{T_\pgd}^2}{2\eta T_\pgd} + \eta\left[L^2 + \beta^2\gamma\delta_0^2\right] &\leq \frac{2\gamma\delta_0^2}{\eta T_\pgd} + \eta[L^2 + \beta^2\gamma\delta_0^2] \\
      &= 2\sqrt{\frac{2\gamma\delta_0^2(L^2 + \beta^2\gamma\delta_0^2)}{T_\pgd}},
  \end{align*}
  from which we obtain the desired bound.
\end{proof}


==> results/nonlinear/perf/srcTrainBound.tex <==
\begin{restatable}[Source Training Bound]{lemma}{srcTrainBound}
  \label{lemma:nonlin-src-train-bound}
  Let $\theta \in \Theta_0$ be a minimizer of the training objective in \eqnref{eqn:adaptation-src-proc-general}.
  Then, with probability at least $1 - \delta$ over the random draw of inputs and labels,
  \[
    \frac{1}{T}\sum_{t \in [T]}\inf_{g_t \in \adaptset_\theta^{\constraintset_\source}}\meanloss_{\infty}^{g_t^\ast}(g_t) - \meanloss_{\infty}^{g_t^\ast}(g_t^\ast) \lesssim \frac{1}{\delta T}\mathcal{R}_{n_\source}\left[\Union_{\theta \in \Theta_0}\left(\adaptset_\theta^{\constraintset_\source}\right)^{\otimes T}\right] + \frac{B}{\delta\sqrt{n_\source T}}.
  \]
\end{restatable}
\begin{proof}
  For any $t \in [T]$, we define the empirical risk minimizer $\bar{g}_t \defas \argmin_{g \in \adaptset_\theta^{\constraintset_\source}}\meanloss^{g_t^\ast}(g)$.
  Then, since $\theta$ minimizes the training objective in \eqnref{eqn:adaptation-src-proc-general},
  \[
    \sum_{t \in [T]}\meanloss^{g_t^\ast}(\bar{g}_t) - \meanloss^{g_t^\ast}(g_t^\ast) \leq 0.
  \]
  Following the canonical risk decomposition, we have that
  \begin{align*}
    \sum_{t \in [T]}\meanloss_{\infty}^{g_t^\ast}(\bar{g}_t) - \meanloss_{\infty}^{g_t^\ast}(g_t^\ast) &\leq \sum_{t \in [T]}\meanloss_{\infty}^{g_t^\ast}(\bar{g}_t) - \meanloss^{g_t^\ast}(\bar{g}_t) + \sum_{t \in [T]}\meanloss^{g_t^\ast}(\bar{g}_t) - \meanloss^{g_t^\ast}(g_t^\ast) \\
      &\qquad + \sum_{t \in [T]}\meanloss^{g_t^\ast}(g_t^\ast) - \meanloss_{\infty}^{g_t^\ast}(g_t^\ast) \\
      &\leq 2\sup_{\substack{\theta \in \Theta_0 \\ g_t \in \adaptset_{\theta}^{\constraintset_\source}}}\abs{\sum_{t \in [T]}\meanloss_\infty^{g_t^\ast}(g_t) - \meanloss^{g_t^\ast}(g_t)}.
  \end{align*}

  We give a high-probability bound on the right-hand side by first bounding its expectation, and then applying Markov's inequality to obtain the desired result.
  To bound the expectation, note that via symmetrization,
  \[
    \expt{\sup_{\substack{\theta \in \Theta_0 \\ g_t \in \adaptset_{\theta}^{\constraintset_\source}}}\abs{\sum_{t \in [T]}\meanloss_\infty^{g_t^\ast}(g_t) - \meanloss^{g_t^\ast}(g_t)}} \leq 2\expt{\sup_{\substack{\theta \in \Theta_0 \\ g_t \in \adaptset_{\theta}^{\constraintset_\source}}}\abs{\frac{1}{n_\source}\sum_{t \in [T]}\sum_{i \in [n_\source]}\epsilon_{ij}\ell(g_t(x_{i, t}), y_{i, t})}}
  \]
  Recentering about $\ell(0, y_{i, t})$ and using the constant-shift property of the Rademacher complexity,
  \begin{align*}
    &\expt{\sup_{\substack{\theta \in \Theta_0 \\ g_t \in \adaptset_{\theta}^{\constraintset_\source}}}\abs{\frac{1}{n_\source}\sum_{t \in [T]}\sum_{i \in [n_\source]}\epsilon_{ij}\ell(g_t(x_{i, t}), y_{i, t})}} \\
      &\quad \leq \expt{\sup_{\substack{\theta \in \Theta_0 \\ g_t \in \adaptset_{\theta}^{\constraintset_\source}}}\abs{\frac{1}{n_\source}\sum_{t \in [T]}\sum_{i \in [n_\source]}\epsilon_{ij}[\ell(g_t(x_{i, t}), y_{i, t}) - \ell(0, y_{i, t})]}} + B\sqrt{\frac{T}{n_\source}}
  \end{align*}
  Finally, since the loss is $1$-Lipschitz, we can apply the Rademacher contraction principle, from which we find that
  \begin{align*}
    &\expt{\sup_{\substack{\theta \in \Theta_0 \\ g_t \in \adaptset_{\theta}^{\constraintset_\source}}}\abs{\frac{1}{n_\source}\sum_{t \in [T]}\sum_{i \in [n_\source]}\epsilon_{ij}[\ell(g_t(x_{i, t}), y_{i, t}) - \ell(0, y_{i, t})]}} \\
      &\qquad \lesssim \expt{\sup_{\substack{\theta \in \Theta_0 \\ g_t \in \adaptset_{\theta}^{\constraintset_\source}}}\abs{\frac{1}{n_\source}\sum_{t \in [T]}\sum_{i \in [n_\source]}\epsilon_{ij}g_t(x_{i, t})}} = \mathcal{R}_{n_\source}\left[\Union_{\theta \in \Theta_0}\left(\adaptset_\theta^{\constraintset_\source}\right)^{\otimes T}\right].
  \end{align*}
  Putting everything together, we can thus bound the expectation of the maximum deviation as
  \[
    \expt{\sup_{\substack{\theta \in \Theta_0 \\ g_t \in \adaptset_{\theta}^{\constraintset_\source}}}\abs{\sum_{t \in [T]}\meanloss_\infty^{g_t^\ast}(g_t) - \meanloss^{g_t^\ast}(g_t)}} \lesssim \mathcal{R}_{n_\source}\left[\Union_{\theta \in \Theta_0}\left(\adaptset_\theta^{\constraintset_\source}\right)^{\otimes T}\right] + B\sqrt{\frac{T}{n_\source}}.
  \]
  Therefore, by applying Markov's inequality, we have that with probability at least $1 - \delta$,
  \begin{align*}
    \frac{1}{T}\sum_{t \in [T]}\meanloss_{\infty}^{g_t^\ast}(\bar{g}_t) - \meanloss_{\infty}^{g_t^\ast}(g_t^\ast) &\lesssim \frac{1}{T}\sup_{\substack{\theta \in \Theta_0 \\ g_t \in \adaptset_{\theta}^{\constraintset_\source}}}\abs{\sum_{t \in [T]}\meanloss_\infty^{g_t^\ast}(g_t) - \meanloss^{g_t^\ast}(g_t)} \\
      &\lesssim \frac{1}{\delta T}\mathcal{R}_{n_\source}\left[\Union_{\theta \in \Theta_0}\left(\adaptset_\theta^{\constraintset_\source}\right)^{\otimes T}\right] + \frac{B}{\delta\sqrt{n_\source T}}. \qedhere
  \end{align*}
\end{proof}


==> results/optimization/pgdApproximateConvexity.tex <==
\begin{restatable}[Approximate convexity in $\Theta$]{lemma}{pgdApproximateConvexity}
  \label{lemma:pgd-approximate-convexity}
  Let $\theta_1, \theta_2 \in \Theta$.
  Then,
  \[
    \inprod{\grad[\theta]\meanloss(\theta_1), \theta_2 - \theta_1} \leq \meanloss(\theta_2) - \meanloss(\theta_1) + 4\alpha\beta D^2.
  \]
\end{restatable}
\begin{proof}
  Note that $\meanloss$ is a convex function of the vector of predictions $g_\theta(X)$, as it is a sum of convex functions by \assumpref{assump:pgd-loss-assumptions}.
  Therefore,
  \[
    \meanloss(\theta_2) - \meanloss(\theta_1) \geq \inprod{\grad[g]{\meanloss(g_{\theta_1}(X))}, g_{\theta_2}(X) - g_{\theta_1}(X)}.
  \]
  Furthermore, by the chain rule,
  \[
    \inprod{\grad[\theta]\meanloss(\theta_1), \theta_2 - \theta_1} = \inprod{\grad[g]\meanloss(g_{\theta_1}(X)), [\grad[\theta]g_{\theta_1}(X)](\theta_2 - \theta_1)}.
  \]
  Putting the two statements together and applying Cauchy-Schwarz,
  \begin{align*}
    &\meanloss(\theta_2) - \meanloss(\theta_1) - \inprod{\grad[\theta]\meanloss(\theta_1), \theta_2 - \theta_1} \\
      &\quad \geq \inprod{\grad[g]{\meanloss}(g_{\theta_1}(X)), g_{\theta_2}(X) - g_{\theta_1}(X) - [\grad[\theta]g_{\theta_1}(X)](\theta_2 - \theta_1)} \\
      &\quad \geq -\norm[2]{\grad[g]{\meanloss(g_{\theta_1}(X))}}\norm[2]{g_{\theta_2}(X) - g_{\theta_1}(X) - [\grad[\theta]g_{\theta_1}(X)](\theta_2 - \theta_1)} \\
      &\quad \geq -\frac{\alpha}{\sqrt{n}}\norm[2]{g_{\theta_2}(X) - g_{\theta_1}(X) - [\grad[\theta]g_{\theta_1}(X)](\theta_2 - \theta_1)}
  \end{align*}
  Now, by Taylor's theorem, there exists $\bar\theta = \lambda\theta_1 + (1 - \lambda)\theta_2$ such that
  \[
    g_{\theta_2}(X) - g_{\theta_1}(X) - \grad[\theta]g_{\theta_1}(X)(\theta_2 - \theta_1) = [(\theta_2 - \theta_1)^\top\grad[\theta]^2g_{\bar\theta}(x_i)(\theta_2 - \theta_1)]_{i \in [n]}.
  \]
  Consequently, by rearranging,
  \begin{align*}
    \inprod{\grad[\theta]\meanloss(\theta_1), \theta_2 - \theta_1} &\leq \meanloss(\theta_2) - \meanloss(\theta_1) + \frac{\alpha}{\sqrt{n}}\sqrt{\sum_{i \in [n]}[(\theta_2 - \theta_1)^\top\grad[\theta]^2g_{\bar\theta}(x_i)(\theta_2 - \theta_1)]^2\vphantom{\sum^T}} \\
      &\leq \meanloss(\theta_2) - \meanloss(\theta_1) + 4\alpha\beta D^2. \qedhere
  \end{align*}
\end{proof}


==> results/optimization/pgdGradientBound.tex <==
\begin{restatable}[Gradient bound in $\Theta$]{lemma}{pgdGradientBound}
  \label{lemma:pgd-gradient-bound}
  For any $\theta \in \Theta$, we have that
  \[
    \norm[2]{\grad[\theta]\meanloss(\theta)}^2 \lesssim \alpha^2(L^2 + \beta^2 D^2)
  \]
\end{restatable}
\begin{proof}
  Using the Lipschitz assumption in \assumpref{assump:pgd-loss-assumptions},
  \begin{align*}
    \norm[2]{\grad[\theta]\meanloss(\theta)}^2 &= \norm[2]{[\grad[\theta]g_\theta(X)]^\top\grad[g]\meanloss(g_\theta(X))}^2 \leq \norm[F]{\grad[\theta]g_\theta(X)}^2\norm[2]{\grad[g]\meanloss(g_\theta(X))}^2 \\
      &\leq \frac{\alpha^2}{n}\sum_{i \in [n]}\norm[2]{\grad[\theta]g_\theta(x_i)}^2
  \end{align*}
  Now, by integrating, we have that for any fixed $i \in [n]$,
  \[
    \grad[\theta]g_\theta(x_i) = \grad[\theta]g_{0}(x_i) + \left[\int_{0}^{1}\grad[\theta]^2g_{\alpha\theta}(x_i) \ \diff{\alpha}\right]\theta.
  \]
  Therefore,
  \begin{align*}
    \norm[2]{\grad[\theta]\meanloss(\theta)}^2 &\lesssim \frac{\alpha^2}{n}\sum_{i \in [n]}\norm[2]{\grad[\theta]g_{0}(x_i)}^2 + \frac{\alpha^2}{n}\norm[2]{\int_{0}^{1}\grad[\theta]^2g_{\alpha\theta}(x_i) \ \diff{\alpha}}^2\norm[2]{\theta}^2 \\
      &\leq \frac{\alpha^2}{n}\sum_{i \in [n]}\norm[2]{\grad[\theta]g_{\theta_0}(x_i)}^2 + \frac{\alpha^2 D^2}{n}\int_{0}^{1}\frac{1}{n}\sum_{i \in [n]}\norm[2]{\grad[\theta]^2g_{\alpha\theta}(x_i)}^2 \ \diff{\alpha} \\
      &\leq \alpha^2(L^2 + \beta^2D^2). \qedhere
  \end{align*}
\end{proof}


==> results/optimization/pgdPerformanceBound.tex <==
\begin{restatable}[Bound on PGD performance]{theorem}{pgdPerformanceBound}
  \label{thm:pgd-performance-bound}
  Assume we run projected gradient descent on $\meanloss$ with constraint set $\Theta$ for $T_\pgd$ iterations with step size $\eta$ given by
  \[
    \eta = \frac{1}{\sqrt{T_\pgd}}\left(\frac{D}{\alpha\sqrt{L^2 + \beta^2 D^2}}\right).
  \]
  Let $(\theta_t)_{t \in [T_\pgd]}$ denote the sequence of PGD iterates obtained, where $\theta_0 = 0$.
  Then, for any $\theta \in \Theta$,
  \[
    \min_{t}\meanloss(\theta_t) - \meanloss(\theta) \lesssim \alpha\beta D^2 + \alpha D\sqrt{\frac{L^2 + \beta^2 D^2}{T_\pgd}}.
  \]
\end{restatable}
\begin{proof}
  For any $t \in [T_\pgd]$,
  \begin{align*}
    r_{t + 1}^2 &= \norm[2]{\theta_{t + 1} - \theta}^2 \\
      &\leq \norm[2]{\theta_t - \eta\grad[\theta]\meanloss(\theta_t) - \theta}^2 \\
      &= r_t^2 + 2\eta\inprod{\grad[\theta]\meanloss(\theta_t), \theta - \theta_t} + \eta^2\norm[2]{\grad[\theta]\meanloss(\theta_t)}^2 \\
      &\leq r_t^2 + 2\eta\left[\meanloss(\theta_0 + \delta) - \meanloss(\theta_0 + \delta_t) + 4\alpha\beta D^2\right] + \eta^2\alpha^2\left[L^2 + \beta^2D^2\right],
  \end{align*}
  where the first inequality follows from the nonexpansive property of projections onto convex sets.
  Furthermore, the last inequality makes use of the approximate convexity property from \lemmaref{lemma:pgd-approximate-convexity} and the gradient bound over $\Theta$ from \lemmaref{lemma:pgd-gradient-bound}.
  Therefore, via telescoping,
  \[
    r_{T_\pgd}^2 \leq r_0^2 + 2\eta\left[\sum_{t = 0}^{T_\pgd - 1}\meanloss(\theta) - \meanloss(\theta_t)\right] + 8\eta T_\pgd\alpha\beta D^2 + \eta^2T_\pgd\alpha^2[L^2 + \beta^2 D^2],
  \]
  or by rearranging,
  \begin{align*}
    \frac{r_0^2 - r_{T_\pgd}^2}{2\eta T_\pgd} + 4\alpha\beta D^2 + \frac{\eta\alpha^2}{2}\left[L^2 + \beta^2D^2\right] &\geq \frac{1}{T_\pgd}\sum_{t = 0}^{T_\pgd - 1}\meanloss(\theta_0 + \delta_t) - \meanloss(\theta_0 + \delta) \\
      &\geq \min_{t = 0, \dots, T_\pgd - 1}\meanloss(\theta_0 + \delta_t) - \meanloss(\theta_0 + \delta).
  \end{align*}
  Now, using the choice of step size, observe that
  \begin{align*}
    \frac{r_0^2 - r_{T_\pgd}^2}{2\eta T_\pgd} + \frac{\eta}{2}\left[\alpha^2 L^2 + \beta^2D^2\right] &\leq \frac{D^2}{2\eta T_\pgd} + \frac{\eta\alpha^2}{2}[L^2 + \beta^2D^2] \\
      &= \alpha D\sqrt{\frac{L^2 + \beta^2 D^2}{T_\pgd}},
  \end{align*}
  from which the desired claim easily follows.
\end{proof}

